Re-imagining Algorithmic Fairness in India and Beyond

Conventional algorithmic fairness is West-centric, as seen in its sub-groups, values, and methods. In this paper, we de-center algorithmic fairness and analyse AI power in India. Based on 36 qualitative interviews and a discourse analysis of algorithmic deployments in India, we find that several assumptions of algorithmic fairness are challenged. We find that in India, data is not always reliable due to socio-economic factors, ML makers appear to follow double standards, and AI evokes unquestioning aspiration. We contend that localising model fairness alone can be window dressing in India, where the distance between models and oppressed communities is large. Instead, we re-imagine algorithmic fairness in India and provide a roadmap to re-contextualise data and models, empower oppressed communities, and enable Fair-ML ecosystems.

==> ML Fairness India Arxiv 2/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> ML Fairness India Arxiv 2/background.tex <==
\vspace{-2mm}
\section{Background}
\label{sec_background}

Recent years have seen the emergence of a rich body of literature on fairness and accountability in machine learning \eg \cite{barocas2017fairness,mehrabi2019survey}.
% In the recent years, a rich body of research on fairness and accountability in machine learning \cite{barocas2017fairness,mehrabi2019survey} has emerged, aided by the various international conferences and workshops on this topic. 
However, most of this research is framed in the Western context, by researchers situated in Western institutions, for mitigating social injustices prevalent in the West, using data and ontologies from the West, and implicitly imparting Western values, \eg in the premier FAccT conference, of the 138 papers published in 2019 and 2020, only a handful of papers even mention non-West countries, and only one of them---Marda's paper on New Delhi's predictive policing system\cite{marda2020data}---substantially engages with a non-Western context.

%\footnote{\cite{washington2020whose} merely mentions the aftermath of Twitter CEO Jack Dorsey's meeting with Dalit community leaders in India in 2018, as an example of how corporate ethics codes fail marginalized communities. \cite{pujol2020fair} uses the apportionment problem of representatives to the Indian Parliament's Lower House as one of the three problems where they apply their proposed fair allocation algorithm. \cite{celis2020interventions} uses a dataset of the Indian Institute of Technology Joint Entrance Exam scores to test their method to tackle gender bias.}


\vspace{-2mm}
\subsection{Western Orientation in Fair-ML}

% The lack of non-Western representation in fair-ML research is reflected in the sub-groups, and the legal and philosophical roots.

% \toadd{Para on dimensions focused}.
\subsubsection{Axes of discrimination}
The majority of fairness research looks at racial \cite{lum2016predict,sap2019risk,davidson2019racial,manzini2019black,buolamwini2018gender} and gender biases \cite{bolukbasi2016man,buolamwini2018gender,sun2019mitigating,zhao2017men} in models---two dimensions that dominate the American public discourse. 
% One dominant strain of much algorithmic fairness writing has concerned notions of fairness between (US) black and (US) white subgroups. 
However these categories are culturally and historically situated \cite{hanna2020towards}. Even the categorisation of proxies in fairness analyses have Western biases and origins; \eg{} the Fitzpatrick skin type is often used by researchers as a phenotype \cite{buolamwini2018gender}, but was originally developed to categorise UV sensitivity) \cite{fitzpatrick1988validity}.
While other axes of discrimination and injustices such as disability status \cite{hutchinson2020social}, age \cite{diaz2018addressing}, and sexual orientation \cite{garg2019counterfactual} have gotten some attention, 
% very little research has looked into potential axes of unfairness in other geographies and cultures. For instance, 
biases relevant to other geographies and cultures are not explored (\eg{}Adivasis (indigeneous tribes of South Asia) and Dalits). As \cite{mulligan2019thing} points out, tackling these issues require a deep understanding of the social structures and power dynamics therein, which points to a wide gap in literature. 


\subsubsection{Legal framing}
% Algorithmic fairness research has been heavily influenced by Western and particularly US societal contexts, with a large focus on US state deployments of force (predictive policing and recidivism risk assessment) as well as state regulation of resource allocations (including housing, loans, and education). 
Since early inquiries into algorithmic fairness largely dealt with US law enforcement (predictive policing and recidivism risk assessment) as well as state regulations (\eg{}in housing, loans, and education), the research framings often rely implicitly on US laws such as the Civil Rights Acts and Fair Housing Act, as well as on US legal concepts of discrimination. Indeed, researchers since the late 1960s have tried to translate US anti-discrimination law into statistical metrics \cite{hutchinson201950}. 
The community also often repurposes terminology from US legal domains, such as ``disparate impact'', ``disparate treatment'', and ``equal opportunity'',
% (although others such as \cite{lipton2018does} 
% have explicitly tried to use non-legal phrases),
or use them as points of triangulation, in order to compare technical properties of fairness through analogy with legal concepts \cite{green2020algorithmic, green2020false}.
% Fairness research is often fond of repurposing terminology from US legal domains, such as ``disparate impact'', ``disparate treatment'', ``equal opportunity'' (although others such as \cite{lipton2018does} have explicitly tried to use non-legal phrases). In other cases, US legal concepts are used as a point of triangulation, in order to compare technical properties of fairness through analogy with legal concepts (e.g. \cite{green2020algorithmic, green2020false}.
% 
% https://arxiv.org/pdf/1811.10104.pdf
% Ben Greene paper
% Ben and Meg's History paper
% How gender and race may manifest in the Est is different than in the West. 
% 
% 

\subsubsection{Philosophical roots}
% In addition to attempted connections with law, algorithmic fairness has sought to centre itself in Western history of ideas around political philosophy \cite{kohli2018translation}. 
Connections have been made between algorithmic fairness and Western concepts such as egalitarianism \cite{binns2018fairness}, consequentialism \cite{roff2020expected, mulligan2019thing}, deontic justice \cite{binns2018fairness, mulligan2019thing}, and Rawls' distributive justice \cite{mulligan2019thing, joseph2016rawlsian}.
%(It is quipped that Rawls is machine learning's favorite philosopher.)
Indeed, notions of algorithmic fairness seem to fit within a broad arc of enlightenment and post-enlightenment thinking, including in actuarial risk assessment \cite{ochigame2020}. Dr. B. R. Ambedkar's ((1891–1956), fondly called Babasaheb, the leader and dominant ideological source of today's Dalit politics) anti-caste movement was rooted in social justice, distinct from Rawl's distributive justice \cite{rodrigues2011justice} (also see Sen's critique of Rawl's idea of original position and inadequacies of impartiality-driven justice and fairness \cite{sen2009idea}).
% 
Fairness' status as the {\em de facto} moral standard of choice and signifier of justice, is itself a sign of cultural situatedness.
% Challenging globalized modes of fairness, political scientist Sohail Inayatullah argues that Islamic societies exhibit a tension between justice and fairness: i.e., between retributive justice that deals with the fight against injustice, and distributional justice, that focuses on creating a caring society \cite{inayatullah2006culture}.
%
%There is also the story of American philosopher Mortimer Adler attending an international conference eager to engage Asian scholars in a dialogue on the ``\textit{great ideas}'' of justice and freedom, but found to his dismay that ``\textit{all they wanted to talk about, he reported, was harmony!}'' \cite{porter2006globalization}.
%
Other moral foundations \cite{graham2013moral} of cultural importance may often be overlooked by the West, including purity/sanctity.
Traditional societies often value {\em restorative justice}, which emphasises repairing harms \cite{boyes2014suffolk}, rather than fairness, \eg{}contemporary Australian Aboriginal leaders emphasise reconciliation rather than fairness in their political goals \cite{inayatullah2006culture}. 
Furthermore, cultural relationships such as power distance, and temporal orientation, are known to mediate the importance placed on fairness  \cite{lund2013culture}.

% Fairness' status as the {\em de facto} moral standard of choice and signifier of justice, is itself a sign of cultural situatedness.
% % Fairness' status in the FAccT community as the {\em de facto} both i) moral standard of choice and ii) signifier of justice, is itself a sign of cultural situatedness.
% Challenging globalized modes of fairness, political scientist Sohail Inayatullah has argued that in Islamic notions of justice and fairness  (specifically the goals of fighting injustice and creating a caring society) are in tension (Inayatullah, 2006).
% American Western philosopher Mortimer Adler attended an international conference eager to engage Asian scholars in a dialogue on the ``\textit{great ideas}'' of justice and freedom, but found to his dismay that ``\textit{all they wanted to talk about, he reported, was harmony!}'' (Porter, 2006).
% Other Moral Foundations (Graham et al., 2013) may be given cultural importances often overlooked by the West, including purity/sanctity; for example Malaysian Muslim scholar Hadi Akbar Dahlan has considered the question of whether AI should be allowed to decide whether food is {\em halal} (Dahlan, 2018). 
% Traditional societies often value {\em restorative justice}, which emphasises repairing harms (Diamond, 2013), rather than fairness, which leads contemporary Australian Aboriginal leaders to emphasise reconciliation rather than fairness in their political goals (Inayatullah, 2006). 
% Furthermore, cultural relationships within a society are known to mediate the importance that people place on fairness, with power distance, long-term orientation and cultural exposure all moderating the importance that subjects place on both outcome fairness and procedural fairness (Lund et al., 2013).

%\noindent \toadd{Extra space. Use this wisely. Don't overflow to the next page.\hfill}
%\noindent \toadd{Extra space. Use this wisely. Don't overflow to the next page.\hfill}

\vspace{-2mm}
\subsection{Fairness perceptions across cultures}
% \subsection{Translating notions from Global North to South}
% Here, we can summarize literature (STS, Philosophy, etc.) on attempts to translate related concepts like fairness, justice, privacy, ethics etc. to the East or India in particular. There is some literature already that I found, but there must be more. This discussion could be framed as literature to learn from, having done in other contexts what we are setting out to do for ML fairness.

% Social Psychology
Social psychologists have argued that justice and fairness require a lens that go beyond the Euro-American cultural confines \cite{leung2001social}.
% have long studied how perceptions of justice and fairness vary across cultures and how those variations impact the operationalizations of fairness in those societies \cite{leung2001social}. 
While the concern for justice has a long history in the West (\eg{}Aristotle, Rawls) and the East (\eg{}Confucius, Chanakya), they show that the majority of empirical work on social justice has been situated in the US and Western Europe, grounding the understanding of justice in the Western cultural context. 
% Universal applications of justice and fairness require a lens that go beyond the Euro-American cultural confines. 
% Social psychology inquiries into cross-cultural differences in justice and fairness uses the individualism versus collectivism framework, as well as the notion of power distance (roughly, egalitarian vs. hierarchical). 
Summarising decades worth of research, \cite{leung2001social} says that the more collectivist and hierarchical societies in the East differs from the more individualistic and egalitarian cultures of the West in how different forms of justice---distributive, procedural, and retributive---are conceptualised and achieved. 
For instance, \cite{blake2015ontogeny} compared the acquisition of fairness behaviour in seven different societies: Canada, India, Mexico, Peru, Senegal, Uganda, and the USA, and found that while children from all cultures developed aversion towards disadvantageous inequity (avoid receiving less than a peer), advantageous inequity aversion (avoid receiving more than a peer) was more prevalent in the West.
Similarly, a study of children in three different cultures found that notions of distributive justice are not universal: ``children from a partially hunter-gatherer, egalitarian African culture distributed the spoils more equally than did the other two cultures, with merit playing only a limited role'' \cite{schafer2015fair}. 
See above point on Dr. B. R. Ambedkar's centring on priority-based social justice for caste inequalities.
% Traditional societies also value fairness differently; a study of children in three different cultures found that notions of distributive justice are not universal: ``children from a partially hunter-gatherer, egalitarian African culture distributed the spoils more equally than did the other two cultures, with merit playing only a limited role'' \cite{schafer2015fair}. 
The above works point to the dangers in defining fairness of algorithmic systems based solely on a Western lens.


\vspace{-2mm}
\subsection{Algorithmic fairness in the non-West}% Here we summarize existing literature situated in the Indian context. It would be great if we can highlight instances where such literature attempts to simply apply the Western derived notions on fairness directly into the Indian context without reconciliations of values/culture at some level. If this turns out to be the case, it might be an even more compelling argument in favor of our paper.
The call for a global lens in AI accountability is not new \cite{paul2018reflecting,hagerty2019global}, but the ethical principles in AI are often interpreted, prioritised, contextualised, and implemented differently across the globe \cite{jobin2019global}. Recently, the IEEE Standards Association highlighted the monopoly of Western ethical traditions in AI ethics, and inquired how incorporating Buddhist, Ubuntu, and Shinto-inspired ethical traditions might change the processes of responsible AI \cite{ieeeglobal2019}.
%\footnote{\url{https://standards.ieee.org/content/dam/ieee-standards/standards/web/documents/other/ead1e_classical_ethics.pdf}} 
Researchers have also challenged the normalisation of Western implicit beliefs, biases, and issues in specific geographic contexts; \eg{}India, Brazil and Nigeria \cite{sambasivan2018toward}, and China and Korea \cite{shin2019toward}.
Representational gaps in data is documented as one of the major challenges in achieving responsible AI from a global perspective \cite{arora2016bottom,shankar2017no}. For instance, \cite{shankar2017no} highlights the glaring gaps in geo-diversity of open datasets such as ImageNet and Open Images that drive much of the computer vision research. \cite{agarwal2020entity} shows that NLP models disproportionately fail to even detect names of people from non-Western backgrounds.

\vspace{-2mm}
\subsection{Accountability for unfairness}
%Fairness is the dominant theme of the FAccT conferences, as seen from FAccT2020's having eight paper sessions dedicated to fairness, sensitive attributes and auditing, compared to a single session on accountability. However 
Discussion of accountability is critical to any discussions of fairness, \ie{}how do we hold deployers of systems accountable for unfair outcomes?
Is it fair to deploy a system that lacks in accountability? Accountability is fundamentally about answerability for actions \cite{kohli2018translation}, and central to these are three phases by which an actor is made answerable to a forum: information-sharing, deliberation and discussion, and the imposition of consequences  \cite{wieringa2020account}. 
Since outcomes of ML deployments can be difficult to predict, proposals for accountability include participatory design \cite{katell2020toward} and participatory problem formulation \cite{martin2020participatory}, sharing the responsibility for designing solutions with the community. 
% one approach has been mechanisms of accountability at the design phase, such as participatory design \cite{katell2020toward}. 
% In this way, responsibility for the design is shared with the community.
%In fact, concepts of responsibility and accountability are intertwined in Western philosophy; under one account they are hybridised thus: ``attributability-responsibility assessments respond to facts about an agent’s character, accountability-responsibility responds to an agent’s degree of regard for others, and answerability-responsibility responds to an agent’s evaluative judgments'' \cite{shoemaker2011attributability}.
%These concepts are held distinct from that of liability, which may not require moral fault \cite{nissenbaum1996accountability}.
Nissenbaum distinguishes four barriers to responsibility in computer systems: (1) the problem of many hands, (2) bugs, (3) blaming the computer, and (4) ownership without liability \cite{nissenbaum1996accountability}.
These barriers become more complicated when technology spans cultures: more, and more remote, hands are involved; intended behaviours may not be defined; computer-blaming may meet computer-worship head on (see Section~\ref{sec_findings}); and questions of ownership and liability become more complicated.

% The need for a global lens in AI accountability has been put forth by international agencies such as USAID \cite{paul2018reflecting} as well as within academic circles \cite{hagerty2019global}.
% \cite{jobin2019global} observes a global convergence emerging around the ethical principles in AI, but with differences in how they are interpreted, prioritised, contextualised, and implemented. In their report on classical ethics in autonomous and intelligent systems,\footnote{\url{https://standards.ieee.org/content/dam/ieee-standards/standards/web/documents/other/ead1e_classical_ethics.pdf}} the IEEE Standards Association highlights the monopoly of Western ethical traditions in AI ethics, and considers how incorporating Buddhist, Ubundu, and Shinto-inspired ethical traditions might change the processes of responsible AI. 
% % There has also been inquiries situated in specific countries. For instance, 
% \cite{sambasivan2018toward} lays out research provocations for AI for the next billion users --- countries like India, Brazil, and Nigeria that has seen massive growth online, that challenges the implicit beliefs, biases, and issues from the Western contexts that may be normalised in AI. \cite{shin2019toward} studies the social cost of AI in China and Korea from a critical socio-technical lens. 

% Representational gaps in data is documented as one of the major challenges in achieving responsible AI from a global perspective \cite{arora2016bottom,shankar2017no}. For instance, \cite{shankar2017no} highlights the glaring gaps in geo-diversity of open datasets such as ImageNet and Open Images that drive much of the computer vision research.
% % They observe the amerocentric and eurocentric representation bias in ImageNet \cite{} and Open Images \cite{}, two of the most commonly used datasets to train computer vision models, and demonstrate strong performance differences in models trained using these datasets on images from different locales.
% \cite{agarwal2020entity} shows that NLP models disproportionately fail to detect names of people from non-Western background.
% % ; for instance, state-of-the-art models correctly identified 99.7\% of common US names, compared to only around 85\% of Vietnamese and Indonesian names, since standard datasets available to train these models use newswire texts from the West, with very few instances of `foreign' named entities. 

Specific to the Indian context, scholars and activists have outlined opportunities for AI in India \cite{kalyanakrishnan2018opportunities}, proposed policy deliberation frameworks that take into account the unique policy landscape of India \cite{marda2018artificial}, and questioned the intrusive data collection practices through Aadhaar (biometric-based unique identity for Indians) in India \cite{ramanathan2014biometrics,ramanathan2015considering}. Researchers have documented societal biases in predictive policing in New Delhi \cite{marda2020data}, caste \cite{thorat2007legacy} and ethnicity \cite{ChutiaCh43:online} biases in job applications, call-center job callbacks \cite{banerjee2009labor}, caste-based wage-gaps \cite{madheswaran2007caste}, caste discrimination in agricultural loans decisions \cite{kumar2013does}, and even in online matrimonial ads \cite{rajadesingan2019smart}.



% \toadd{Add a para on AI fairness and responsibility conversations in India (citations in comment below in tex file)}

% \toadd{Add a para on specific axes of bias in India such as caste (citations in comment below in tex file) and maybe others?}

\begin{comment}

% Global ML Ethics: A Review of the Social Impacts and Ethical Implications of Artificial Intelligence
% Reflecting the Past, Shaping the Future: Making ML Work for International Development by USMLD
% Classical Ethics in A/IS [See Section 2 — Classical Ethics From Globally Diverse Traditions] by The IEEE Standards Association
% The global landscape of ML ethics guidelines. Jobin et al. 

% Toward fair, Accountable, and Transparent Algorithms: Case Studies on Algorithm Initiatives in Korea and China
% Towards responsible ML for the next billion users by Sambasivan and Holbrook
ML Accountability in the Japanese context by Hatta
How the machine ‘thinks’: Understanding opacity in machine learning algorithms by Burrell (focus on Ghana)
Some Requests for Machine Learning Research from the East African Tech Scene by Cvitkovic (not fairness-specific, is fairness-relevant)

% No Classification without Representation: Assessing Geodiversity Issues in Open Data Sets for the Developing World by Shankar et al
% Arora, P. (2016). The Bottom of the Data Pyramid: Big Data and the Global South. International Journal of Communication, 10, 1681-1699
Fighting poverty with data by Blumenstock


% Opportunities and Challenges for Artificial Intelligence in India by Kalyanakrishnan et al
% Artificial Intelligence Policy in India: A framework for engaging the limits of data-driven decision-making by Marda
% Data in New Delhi’s predictive policing system by Marda on the elaborate human and data biases
% Labor Market Discrimination in Delhi: Evidence from a Field Experiment by A. Banerjee et al
Considering Social Implications of Biometric Registration: A Database Intended for Every Citizen in India [Commentary]. Usha Ramanathan
Biometrics Use for Social Protection Programmes in India Risk Violating Human Rights of the Poor. Usha Ramanathan
Life of a Tuple - NRC in Assam by CIS 
Open governance and surveillance: A study of the national rural employment program in Andhra Pradesh, India by Veeraraghavan
Affirmative Action in Education: Evidence from Engineering College Admissions in India by Bertrand et al
Obtaining a driver’s license in India by Bertrand et al

% Caste discrimination in the Indian labour market by Attewell
% Smart, Responsible, and Upper Caste Only: Measuring Caste Attitudes through Large-Scale Analysis of Matrimonial Profiles by Rajadesingan et al. 
% ‘Caste’ as a social data category and the implications that caste as identity-marker produces for an ML/ML system by Raval



GIS Information Watch ML and Human Rights - goldmine data
Extracting fairness Policies from Legal Documents not much on bias, just Wordnet extractions


\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> ML Fairness India Arxiv 2/changelog.tex <==
Quick Links
Internal Feedback
Interviewee Feedback
Acks

Internal Feedback

Daniel Russel
Overall, an interesting paper that I appreciate, but I feel as though I'm missing a few things. First: Where's this going? What conference do you want to submit this to? Is this an opinion piece? An overview? A featured article? What's the role that you're intending for this article?
Apologies! This is a paper submission for FaccT 2021, formerly FAT*. They have a Human Factors (HCI) track, under which we’re submitting this paper.

While I feel as though it would be a valuable article for the greater community, I think this will need to also be approved by PR before publication.
We have sought approvals from P-counsel, PR, Comms and Policy and already have an LGTM from P-counsel. We’ll update the thread once we get LGTMs from other parties.

A couple of quick comments:

* the summary seems cut off... it ends mid-sentence. Is there supposed to be more there?
In general, the paper has become a lot tighter and has more of a flow since a week ago. These formatting issues have been identified and fixed.

* the copyright notice (page 1) is strange and odd. Woodstock?
Yeah, this is the new ACM sigconf template

* the Mortimer Adler reference is fairly second hand and seems inconsistent with the paper you're trying to write. That story is reported as "the story is told of Mortimer Adler attending.." (I see your point, but that's a slim, dubuious story to base such an essential argument on.)
Thanks for pointing this out. We’ll be on the lookout for a better reference to bring out the ‘justice’ in America vs. ‘harmony’ in the East. For now we’ll scrap this reference.  

* you write that "AI/ML systems tend to be largely open-sourced and openly discussed.." (in Openness), but then write "Our findings point to how several high-stakes decisions are made behind closed doors in India.." (in Public Algorithm Literacy). I think I see what you mean, but both things probably can't be true. (And I'm not even sure that "AI/ML systems tend to be largely open-sourced..." -- there ARE a lot of open-source libraries that are available, but there is also a LOT of non-open-sourced code that's in common use. Do you know of any way to estimate the quantity of each?)
Thanks for pointing this out. The text has changed since then and now we don’t have a mention of open-sourced models. Though originally we didn’t mean it as open source code, but as openly scrutable models and outputs. But I suppose it wasn’t clear :).

* unclear to me how quoting the Zapatistas will help your argument. ("As the Zapatistas said..") The citation is missing, but I don't know how a rhetorical line from a political/miltant group will advance the story you want to tell. Since that section starts with Mbembe's critique of objectivism and goes on to argue for making inclusive knowledge production, you could probably lose that sentence and improve the readability of the section.
This was a bit challenging, as the Zapatista quote is deeply cherished in the decolonial theory circles, which originated in Latin America and saw the Zapatista movement as an indigeneous expression of autonomy. But given the militant implications you rightly point out, we have now removed the sentence. The readability is also better now, going straight to Mbembe.

* the phrase "communism without dictatorship (sanghas) espoused by Dr. B.R. Ambedkar," probably needs a citation. I'm not familiar enough with this to know what you're referring to. (Is this also from [53]?)
Thanks, added now.

* Biggest question: How did you go from your research Method ("interviewing with 36 expert researchers, activists, and lawyers working closely with marginalized Indian communities" then coding those interviews) to the Findings of Section 4? There's no description of the clustering / topic-identification process you followed to determine that these topics ("Missing data," "one-to-one correspondence," "Good data profiles," etc.) were the most important topics that emerged from the interviews with the "researchers, activists, and lawyers." What was that process?
Great point! An obvious miss on my part. New addition in Method: 
“Transcripts were coded and analyzed for patterns using an inductive approach~\cite{Thomas2006general}. From a careful reading of the transcripts, we developed categories and clustered excerpts, conveying key themes from the data. Two team members created a code book based on the themes, with seven top-level categories (sub-group discrimination, data and models, law and policy, biases, AI applications, ML makers, and solutions) and several sub-categories (\eg{}caste, missing data, proxies, consent, algorithmic literacy, and so on). The three power structures that we describe below were then developed and applied iteratively to the codes.”

For instance, in section 4.2, where did Table 1 come from? ("Axes of potential (un)fairness in India") You say that the table is "(by no means exhaustive, but representative of our interview results)." But there's a lot of numeric data there (e.g., caste population sizes)... where did THAT come from? (Later you say it's a composite of your interviews and "desk research" but you're presenting data without citation or sources.)
Thanks for pointing this out. We now have body text saying,
“In Table 1, we present a summary of axes of discrimination in India, derived from interviews and enriched through secondary research and statistics from authoritative sources, to substantiate attributes and proxies.”


Jess Holbrook

Introduction
"We contend that India is on an alternative path to AI, characterised by pluralism, socio-economic development, technocratic nation-building, and unequal AI capital—which requires us to confront many assumptions made in conventional algorithmic fairness." - may want to make explicit what this an alternative to, it is implied but may benefit from being explicit
The "ML makers’ distance:" paragraph was a bit unclear to me. I think you're trying to make two points that might be separated - 1) ML makers are both physically and culturally distant from their users and 2) even when they are close, they are at less influential points in the development pipeline and not in a position to remediate those distances.
"The AI imaginary" - do you mean imagination? 
The "AI aspiration:" paragraph seems like it has two distinct ideas in it - 1) the imagination is aspirational and a consequence is it is being used in high stakes domains, perhaps too early and 2) this aspirational and optimistic nature is in part due to a lack of adequate interrogation of these systems, which requires the right ecosystem of tools, policies, processes, etc.
Table 1
Colonial law 377 traces - I'm not familiar with this one but just might be me. Calling out that it may not be 100% clear to readers what this means.
4.2 ML makers' distance
"Many respondents shared how street-level bureau-crats, administrative offices, and front line workers—the human infrastructures who played a crucial role in providing recourse to marginalised Indian communities—were removed in ML systems." - I love insights like this. So good.
5.1.1 Data Considerations
"when data is neither replicable nor reproducible, what conditions can we set to expect reliability?" - I wasn't sure what this meant
I may have missed it but do you call for more open data sets in this section? That would go a long way with transparency and you could link it to projects like the Lacuna Fund and how these datasets can enable local developer ecosystems. It could go in 5.3 as well. 
Alex Hanna:
Thanks for this paper, Nithya and Vinod. It's really insightful and revealing. I have some general comments on this paper, and then some more specific recommendations for other references. My more general comments are that this paper is doing a lot. I think the critique of the Western-centric notions of fairness and fair-ML are all on point, and Table 1 is really helpful for this. My more specific version of the comments are mostly around Section 5, which I think points to many directions for future action, but is also very ambitious insofar as who is going to adopt these suggestions. For instance, is this targeted towards fair-ML people, or AI practitioners writ large? Is this targeted towards participatory partners? I think sharpening the imaginary audience can help prioritize which of the recommendations you'd like to dig into in deep detail. Because I'm interested most in data infrastructure, I find that I want more there, bu I think the considerations of empowerment would appeal more to design-forward scholars and practitioners, and openness perhaps to model builders.
 
More specifically, some thoughts and references which can be helpful --
 
There's some ethnographic work by STSer Ranjit Singh on Aadhaar which could be relevant here --
- https://dl.acm.org/doi/10.1145/3025453.3025910
- https://www.tandfonline.com/doi/abs/10.1080/00856401.2019.1602810?journalCode=csas20
 
There's a connection of "document poverty" to Dean Spade's idea of administrative violence and the mismatch of one's identity docs, especially for trans people.
 
"Optimization strategies in algorithmic fairness, such as equal opportunity or equal odds, stem from epistemologies and legalities of the United States."
- I'd also say they are based in a "perpetrator-based" perspective, rather than "victim-based" one, which has been critiqued by critical race scholarship (cf. Alan Freeman). The rights-based perspective has always been narrowly "white", to be blunt. Also see Dean Spade on this.
 
"In India, the strong aspiration for social and economic upliftment was also reported to be accompanied by unquestioning trust in automation and minimal checks and balances."
- Lilly Irani's book might be a good reference here: https://www.google.com/books/edition/Chasing_Innovation/tbZuDwAAQBAJ?hl=en&gbpv=1&printsec=frontcover
 
Reena:

Comments provided in-line here.

Martin
Hi Nithya,
 
Sounds like an impressive set of work, and thanks for sending that paper--very interesting! Yes, please do send the latest research agenda doc.
 
Super-dumb question on the paper: what's the difference between "Indic" and "Indian"?
 
Open-ended question: the paper describes quotas (reservations) as an Indic approach to fairness, different from the US. But the US has a long history of quota systems. Of course, some types of quotas are currently illegal, but not all of them (to give just one example, today government contracts have to go to a certain percentage of businesses owned by minorities/women/veterans). Historically, quotas have been used in the US for a long time... in the New Deal in the 30s, some agencies had to give a certain percentage of jobs to Black workers. At the same time, there were also notorious quotas that put a cap on minorities (e.g., on Jewish applicants to elite colleges, for a while, allowing no more than something like 15%). So quotas are definitely a very familiar (if controversial) technique in the US. Is the difference in India that they're always legal, and people support them without any controversy? 

--Martin



Feedback on paper from interviewees: 
Ranjit:
The last sentence of Missing data and invisible humans in Section 4.1.1 Data considerations, which focuses on trust in data workers requires more nuance. I believe the story is more complicated than placing trust in data workers. There have also been situations when data workers have entered data incorrectly without actual conversations with people affected by changes in their data records. As a result, there have been social movements in India organized by the Right to Information activists (MKSS, more specifically) on securing representation through data along with calls for Janata Information Systems. See also the attached paper. 
In the same section, when talking about Axes of un-fairness, harms, and discriminatory proxies, another issue to consider is literacy and how it constrains the ability of a person in becoming digitally-rich as already indicated in the first paragraph of Section 4.1.2 Model Considerations.
Section 4.2 ML Markers' distance ends with a discussion on developers of AI belonging to privileged castes and middle-class backgrounds, but it ends in a quote talking about "white male problem of tech". To me, it felt kind of jarring because the developers referred to in the paragraph are not typically "white." It seemed to me like a conflation of two different problems of contending with race and caste that are similar but not the same. 
Savita:
- In addition to opening up the research & policy debates, would you hope for a set of principles specific to country contexts? In doing so, is that acknowledging that some principles are not universal?
- you mention the AI imaginary is aspirational. It might be worth clarifying all the stakeholders for whom it's aspirational (you mention initiatives but are they led by any particular driver?)
- In research ethics, you talk about being careful on consent, storing documentation safely etc. You also acknowledge yourselves as privileged (a nice touch!) but is it worth making the link between the two more explicit by saying something like you acknowledge these are your interpretations of research ethics, which may also not always be universal? Don't know if that is too risky to say!
 
Aneesh:
Good to hear from you. The paper looks wonderful. I have only one citation idea, my 2006 book, Virtual Migration :-). It was the first work (apart from my 2001 dissertation) to talk about algorithmic power; it developed the whole theory of algocracy. 
 
Murali:
Thanks for the patience, and I am attaching my comments/observations. Some are more pertinent than others. I am aware that this delay is not ideal, but I hope this is still useful to authors.
Two general comments:
As happens in the race and technology domain where collaboration with black scholars is a valued as a sign of ethical and political position, I sincerely hope future discussions about building caste-sensitive include Dalit and anti-caste scholars/activists. I am confident that authors will move towards that direction in their next phase.
This exciting paper has a lot of scopes to refer to Dalit and Adivasi scholarships (e.g., feminist/poco/media-cultural critiques) and in turn, could benefit from their critical insights. After all, each citation is political.
 
Follow-up from Murali
Last week, I gave a talk on "Caste in legal regimes" at King's India Institute: I argued how "unconventional legal regimes" - on sites such as the Internet - are now replacing  "conventional legal regimes."  
 
I presented an analysis of how a western legal doctrine (the impartiality test) - despite well-meaning intentions - might enable casteism on the Internet. I have to find out if they recorded the talk and would upload it.
 
A succinct discussion on the manifestation of "modern caste" (and other relevant non-western categories) and its everyday communicative practice is very relevant to the scope of the paper.
 
As you well know, I am very keen to be part of any future discussions on this topic.Thank you.
Attachments - Bond Caste & Development; Caste Definitions
Best wishes,
Murali
 
PS: do see our arguments related to caste and (lack of) disaggregated data in BOND Caste and Development Report
 
(350 words allowed)
Thanks to the reviewers for their valuable comments. We believe our paper makes a critical contribution to shift the boundaries of the current Western discourse in fairness.

Scope (R3):
Our intention is to set out a research agenda and point to concrete directions one could take. Going into the specifics like solving casteist bias online is beyond the scope of our 10-page paper. We absolutely agree that caste is an important issue, and definitely warrants a paper on its own. So do many other issues we raised: fairness challenges w/ data distortions, or fairness and reservations etc. Our paper sets a research agenda for fair-ML in India that outlines open issues that need in-depth investigations, but also to outline the larger ecosystem considerations one must take into account when doing so (we will clarify).

India specific factors (R1, R3): 
Our paper discusses factors impacting fairness in India -- pronounced in India, and not necessarily unique to India (we state this). India is a globalized country. We do not wish to focus on ‘Indian’ factors in the Western imagination, and exocitize India as the ‘other’ (e.g., tropes of caste, poverty, ancient culture etc.) [ref: Edward Said and numerous decolonial authors we borrow from and cite]. Our Introducton may have contributed to the feedback, with our use of terms like ‘not limited to India alone’ (which we will revise for clarity).

Expert interviews (R2):
This method is common to many social sciences, including HCI where we come from, to understand the landscape when there are no specific systems to gain access to, and to create a systemic analysis, not specific to an intervention.

Broad (R3):
R3’s reading of the paper as broad is correct. The issues are not caused by Fair-ML factors, but impact fairness of models, fairness audit tools, and structures to turn research into reality. We mention that attempting to do Fair-ML without accounting for these broad issues may be futile or even harmful.  To articulate these sociotechnical factors, we deemed it appropriate to engage with diverse experts that work closely with marginalized communities. We will clarify these points further. 

Review #228A3 Dec 2020
Comments for author
This was a well-written, clearly presented paper.
This paper presents interview data from 36 researchers, activists and lawyers working in Indian contexts with marginalised communities. Interviews address the notion of algorithmic fairness, and the extent to which interviewees consider this feasible in light of the community groups they work with.
This is a reasonably good quality paper in terms of its empirical basis. n=36 interviews gives a solid foundation to work with (especially given the nature of the interviewees). The theoretical discussion, and arguments reached are also of a good quality. All in all, this is a good standard of paper.
Clearly written and presented - should be accessible to novice readers, and detailed enough to be of interest to people working directly in the area.
Good use of previous literature. From my own disciplinary b/g this would seem to have too much use of previous literature (194 references is about 154 more than I would expect to see!)
I am not an expert in this literature, but this paper seems to make a contribution to my adjacent knowledge of the academic literature in this area. Given the vastness and complexity of Indian society, I would welcome a clearer sense to what extent the paper can speak to 'Indian' issues, or what regional/caste nuances are being glossed over
Review #228B3 Dec 2020
Comments for author
The paper makes a relevant contribution to the study of algorithmic fairness by de-centering common practices and approaches. I am not persuaded that interviewing experts is the most appropriate method to make the case, but I think the treatment and analysis is sufficiently cogent.
Explanations of the motivation, argument, methods and results are clear and appropriate.
The paper is original in that not many scholars have attempted to achieve this analytical goal in the particular context of India (or the global south).
The paper cites abundant extant literature. It draws on appropriate bodies of work to make the case.
The argument put forth in this paper is a valuable contribution to reflections on algorithmic fairness. It helps to denaturalize common assumptions established in the field.
The contribution centers on core issues for FAccT.
Review #228C
Comments for author
Quality: The paper is well written and adequately cited. Overall, my biggest complaint is that the arguments made are very broadly centered around inequities in technology access and usage in non-western contexts, whereas the paper describes the issues as specific to shortcomings of fair machine learning in India.
Clarity: The arguments made in the paper are clear individually, but collectively, I found the paper difficult to follow. Many of the criticisms made in the paper touched on a wide array of topics: privacy, socioetechnical systems, etc. As a reader it was difficult to see how all of the issues were related to the exact same root cause -- in this case -- fair machine learning scholarship. This confusion is augmented by the breath of experts called on for interviews. They came from a number of disparate areas: "Computer Science, Activism, Law and Public Policy, etc". It would help if the scope of the criticisms in the paper were narrowed, such that more specific arguments could be made.
Originality: Although the paper is the first paper I have seen which addresses issues in the machine learning fairness scholarship that are specific to India, many of the claims made in the paper are not uniquely specific to India, and almost all of these points been cited in other works. For example, this work does a great job challenging downstream usage assumptions, and binary protected attribute assumptions: "Where Fairness Fails: Data, Algorithms, and the Limits of Anti-discrimination Discourse" by Anna Lauren Hoffman.
Significance/Impact: The paper does a great job outlining how many of the assumptions in fair machine learning are western centric, however the paper does not point to a separate body of work which remedies the issue presented. Some alternatives are mentioned, but they are often too-high level for the scope of the problems outlined in section 2. For example, "Building ties with community workers in the ML dataset collection process can be a starting point in creating high quality data, while respecting their situated knowledge. Combining observational research and dataset analysis will help us avoid misreadings of data."
Relevance: I'd say that the work is highly relevant, and that is definitely headed in the correct direction. I agree that one of the major shortcomings of the fairness literature is that the work makes many western-centric assumptions, but these assumptions are also based in power structures that appear differently everywhere, and are not necessarily unique to the western world. Underrepresentation in data being related to socioeconomic status is an issue that also occurs in the western world, and so I feel it would be helpful to frame this paper in terms of more specific Indian issues. Issues of Caste for example, are very unique to an Indian context, it would have been very helpful as a reader if the author could discuss how to better contextualize Caste, for example, in a machine learning context.



1) 
"  delay-tolerant connectivity, low cost devices, text-free interfaces, partnership with civil society  "
you can cite the Digital Green paper.
Gandhi, R., Veeraraghavan, Rajesh., Toyama, K., Ramprasad, V. Digital Green: Participatory Video for Agricultural Extension. Information Technologies & International Development, Vol. 5, Issue 1, pp1-15, Spring 2009. [PDF] 

Our idea there (though not fully developed) was breaking the idea of expertise, and making farmers as the stars (as opposed to having to rely on agri experts)maybe worth mentioning.

2) Veeraraghavan, Rajesh.Dealing with the Digital Panopticon: The Use and Subversion of ICT in an Indian Bureaucracy. IEEE/ACM Int’l Conf. on Information & Communication Technologies for Development, Cape Town, South Africa, December 2013. [PDF]
This maybe also relevant, though this is before the craze about algorithms took over. Particularly the idea of "hiding behind the computer". I had also discussed the politics of algorithms and how sometimes algorithms maybe necessary to avoid local political interference. A complex idea, but not developed :)

3) Another paper with Vivek Srinivasan (who you spoke to) where we asked the question of "direct" cash transfers, and answered. No. These tech systems needed intermediaries.
Vivek, S., Narayanan, R., Chakraborty, D., Veeraraghavan, R., Vardhan, V. Are Technology-enabled Cash Transfers Really 'Direct'? Economic and Political Weekly, July 28, 2018. [PDF] 


==> ML Fairness India Arxiv 2/conclusion.tex <==
\vspace{-2mm}
\section{Conclusion}
As AI becomes global, algorithmic fairness naturally follows. Context matters. We must take care to not copy-paste the western-normative fairness everywhere.   %As the Zapatistas said, \textit{``the world we want is a world in which many worlds fit''} \cite{escobar?}). 
We presented a qualitative study and discourse analysis of algorithmic power in India, and found that algorithmic fairness assumptions are challenged in the Indian context. We found that data was not always reliable due to socio-economic factors, ML products for Indian users sufffer from double standards, and AI was seen with unquestioning aspiration. We called for an end-to-end re-imagining of algorithmic fairness that involves re-contextualising data and models, empowering oppressed communities, and enabling fairness ecosystems. The considerations we identified are certainly not limited to India; likewise, we call for inclusively evolving global approaches to Fair-ML. %Only then can we hope to create equitable pluriverses in this new AI epoch we live in. 

\vspace{-2mm}
\section{Acknowledgements}
Our thanks to the experts who shared their knowledge and wisdom with us: A. Aneesh, Aishwarya Lakshmiratan, Ameen Jauhar, Amit Sethi, Anil Joshi, Arindrajit Basu, Avinash Kumar, Chiranjeeb Bhattacharya, Dhruv Lakra, George Sebastian, Jacki O Neill, Mainack Mondal, Maya Indira Ganesh, Murali Shanmugavelan, Nandana Sengupta, Neha Kumar, Rahul De, Rahul Matthan, Rajesh Veeraraghavan, Ranjit Singh, Ryan Joseph Figueiredo (Equal Asia Foundation), Savita Bailur, Sayomdeb Mukerjee, Shanti Raghavan, Shyam Suri, Smita, Sriram Somanchi, Suraj Yengde, Vidushi Marda, and Vivek Srinivasan, and others who wish to stay anonymous. To Murali Shanmugavelan for educating us and connecting this paper to anti-caste emancipatory politics and theories. To Jose M. Faleiro, Daniel Russell, Jess Holbrook, Fernanda Viegas, Martin Wattenberg, Alex Hanna, and Reena Jana for their invaluable feedback.

%1) Concerned it raises need for country-by-country approach (Sent him new language we sent Will, alleviated this concern)
%Google just makes me nervous because there are certainly other communities for which this will also be true and it's practically impossible for us to adopt so many tailored approaches but on it's own, the work seems strong and adding some language like that may help position this better"

==> ML Fairness India Arxiv 2/discussion.tex <==
\vspace{-2mm}

\section{Towards AI Fairness in India}
%The concerns we raisemay certainly be true of other countries
\begin{figure*}[ht!]
\includegraphics[width=.79\linewidth]{fairnessframework.png}
\caption{Research pathways for Algorithmic Fairness in India.}
\label{fig:Indiaframework}
\end{figure*}

In Section~\ref{sec_findings}, we demonstrated that several underlying assumptions about algorithmic fairness and its enabling infrastructures fail in the Indian context. To meaningfully operationalise algorithmic fairness in India, we extend the spirit of Dr. B.R. Ambedkar's call to action, ``\textit{there cannot be political reform without social reform}'' \cite{ambedkar2014annihilation}. We need to substantively innovate on how to empower oppressed communities and enable justice within the surrounding socio-political infrastructures in India. Missing Indic factors and values in data and models, compounded by double standards and disjuncture in ML, deployed in an environment of unquestioning AI aspiration, face the risk of reinforcing injustices and harms. We need to understand and design for \textit{end-to-end} chains of algorithmic power, including how AI systems are conceived, produced, utilised, appropriated, assessed, and contested in India. We humbly submit that these are large, open-ended challenges that have perhaps not received much focus or are considered large in scope. However, a Fair-ML strategy for India needs to reflect its deeply plural, complex, and contradictory nature, and needs to go beyond model fairness. We propose an AI fairness research agenda in India, where we call for action along three critical and contingent pathways: \textit{Recontextualising}, \textit{Empowering}, and \textit{Enabling}. Figure~\ref{fig:Indiaframework} shows the core considerations of these pathways. The pathways present opportunities for cross-disciplinary and cross-institutional collaboration. While it is important to incorporate Indian concepts of fairness into AI that impacts Indian communities, the broader goal should be to develop general approaches to fairness that reflect the needs of local communities and are appropriate to the local contexts. 
% We describe these opportunities, drawing from feminist and decolonial lenses, based on our study findings below. 

%Our call for action draws inspiration from scholars such as Donna Haraway who asks to `stay with the trouble', so we acknowledge our complicity, while maintaining that the goal is still recuperation \cite{haraway2016staying}, and Bonnie Nardi who argues that it is necessary to innovate not just the technology, but also the logistical and social arrangements \cite{nardi2019design}.

%nonetheless they are important
%end to end impact of AI
%we don't prescribe who should solve the problem
%opportunity for cross-disciplinary collaboration - such an important issue
\vspace{-2mm}
\subsection{Recontextualising Data and Models}

How might existing algorithmic fairness evaluation and mitigation approaches be \textit{recontextualised} to the Indian context, and what novel challenges does it give rise to? %Research on these questions will require contending with both data and model considerations.  

\subsubsection{Data considerations}\hfill\\
Data plays a critical role in measurements and mitigations of algorithmic bias. However, as seen in Section~\ref{sec_findings}, social, economic, and infrastructural factors challenge the reliance on datasets in India. Based on our findings, we outline some recommendations and put forth critical research questions regarding data and its uses in India.  

Due to the challenges to completeness and representation discussed in Section~\ref{sec_findings}, we must be (even more than usual) sceptical of Indian datasets until they are trust-worthy. For instance, how could fairness research handle the known data distortions guided by traditional gender roles? What are the risks in identifying caste in models? Should instances where models are deliberately `confused' (see Section~\ref{sec_findings}) be identified, and if so what should we do with such data? We must also account for data voids \cite{golebiewski2019data} for which statistical extrapolations might be invalid.

The vibrant role played by human infrastructures in providing, negotiating, collecting, and stewarding data points to new ways of looking at data as dialogue, rather than operations. Such data gathering via community relationships lead us to view data records as products of both beholder and the beheld. Building ties with community workers in the AI dataset collection process can be a starting point in creating high quality data, while respecting their situated knowledge. Combining observational research and dataset analysis will help us avoid misreadings of data. 
% As discussed in Section~\ref{sec_background}, information transparency is critical in holding developers of datasets accountable, and accounts need to be made accessible in local languages (and in some cases non-written form, due to the high non-literacy rates in marginalized Indian populations). 
%AI fairness should How might AI fairness research interface with such grassroots infrastructure of data sourcing? 
Normative frameworks (\eg{} perhaps ethics of care \cite{held2006ethics, asaro2019ai,zevenbergen2020}) may be relevant to take into account these social relations.
A related question is how data consent might work fairly in India. One approach could be to create transitive informed consent, built upon personal relationships and trust in data workers, with transparency on potential downstream applications. Ideas like collective consent \cite{MozillaF26:online}, data trusts \cite{Nesta}, and data co-ops may enhance community agency in datasets, while simultaneously increasing data reliability. %Data literacy workshops with marginalized communities may enable informed consent as well as meaningful inclusion into AI, especially as beneficiaries of algorithmic fairness. 

Finally, at a fundamental level, we must question the categories and constructs we model in datasets, and how we measure them. As well as the situatedness of social categories such as gender (cf. \textit{Hijra}) and race \cite{hanna2020towards}, ontologies of affect (sentiment, inappropriateness, etc.), taboos (\textit{Halal}, revealing clothing, etc.), and social behaviours (headshakes, headwear, clothing, etc) are similarly contextual. How do we justify the ``knowing'' of social information by encoding it in data? We must also question if being ``data-driven'' is inconsistent with local values, goals and contexts. When data are appropriate for endemic goals (\eg{} caste membership for quotas), what form should their distributions and annotations take? Linguistically and culturally pluralistic communities should be given voices in these negotiations in ways that respect Indian norms of representation.

\subsubsection{Model and model (un)fairness considerations} \hfill\\
The prominent axes of historical injustices in India listed in Table~\ref{tab_subgroups} could be a starting point to detect and mitigate unfairness issues in trained models (\eg{}\cite{bolukbasi2016man,zhang2018mitigating}), alongside testing strategies, e.g. perturbation testing \cite{prabhakaran2019perturbation}, data augmentation \cite{zmigrod2019counterfactual}, adversarial testing \cite{kurakin2016adversarial}, 
% semantic analysis, 
and adherence to terminology guidelines for oppressed groups, such as \textsc{SIGACCESS}. However, it is important to note that operationalising fairness approaches from the West to these axes is often nontrivial. For instance, personal names act as a signifier for various socio-demographic attributes in India, however there are no large datasets of Indian names (like the US Census data, or the SSA data) that are readily available for fairness evaluations. In addition, disparities along the same axes may manifest very differently in India. For instance, gender disparities in the Indian workforce follow significantly different patterns compared to the West. How would an algorithm made fairer along gender based on datasets from the West be decontextualised and recontextualised for India? 

Another important consideration is how the algorithmic fairness interventions work with the existing infrastructures in India that surrounds decision making processes.
For instance, how do they work in the context of established fairness initiatives such as reservations/quotas? As an illustration, compared to the US undergraduate admission process of selection from a pool of candidates, the undergraduate admissions in India is done through various joint seat allocation processes, over hundreds of programmes, across dozens of universities and colleges that takes into account test scores, ordered preference lists provided by students, as well as various affirmative action quotas \cite{baswana2019centralized}. The quota system gives rise to the problem of matching under distributional constraints, a known problem in economics \cite{kamada2015efficient, goto2017designing, ashlagi2020assignment}, but has not received attention within the FAccT community (although \cite{cotter2019optimization} is related). First-order Fair-ML problems could include representational biases of caste and other sub-groups in NLP models, biases in Indic language NLP including challenges from code-mixing, Indian subgroup biases in computer vision, tackling online misinformation, benchmarking using Indic datasets, and fair allocation models in public welfare.

\vspace{-2mm}
\subsection{Empowering Communities}
Recontextualising data and models can only go so far without participatorily \textit{empowering} communities in identifying problems, specifying fairness expectations, and designing systems. 

\subsubsection{Participatory Fair-ML knowledge systems}\hfill{}\\
Context-free assumptions in Fair-ML, whether in homegrown or international AI systems, can not just fail, but produce harm inadvertently when applied to different infrastructural and cultural systems. As Mbembe describes the Western epistemic tradition, the knowing subject is enclosed in itself and produces supposedly objective knowledge of the world, ``without being part of that world, and he or she is by all accounts able to produce knowledge that is supposed to be universal and independent of context'' \cite{mbembe2015decolonizing}. How can we move away from the `common good' defined by the researcher---the supposedly all-knowing entity who has the expertise and experience necessary to identify what is of benefit to all \cite{nathan2017good}. Humbly creating grassroots commitments with vulnerable communities is an important first step. Our study discusses how caste, religion, and tribe are eluded even within the Indian technology discourse and policy. Modes of epistemic production in Fair-ML should enable marginalised communities to produce knowledge about themselves in the policies or designs. Grassroots efforts like Deep Learning Indaba \cite{dlindaba}
% \footnote{\url{https://deeplearningindaba.com/2020/}} 
and Khipu \cite{khipu}
% \footnote{\url{https://github.com/khipu-ai}} 
are exemplar of bootstrapping AI research in communities. Initiatives like Design Beku \cite{designbeku}
% \footnote{\url{https://designbeku.in/}} 
and SEWA \cite{sewa}
% \footnote{\url{http://www.sewa.org/}} 
are excellent decolonial examples of participatorily co-designing with under-served communities. 
%Pluriverses \cite{escobar2011encountering} of values in algorithmic fairness can come from justice systems of priority-based social justice by Dr. B. R. Ambedkar \cite{davidlelyveld}, indigenous justice of Adivasis \cite{xaxa2011tribes}, or \textit{dharma} (social ethic) and \textit{karma} (action) from Hinduism\footnote{Hindu concepts may be rejected by Dalits for reinforcing hierarchy \cite{narayanan2001water}}, for example. 


%TODO
\subsubsection{Low-resource considerations} \hfill\\
India's heterogeneous literacies, economics, and infrastructures mean that Fair-ML researchers' commitment should go beyond model outputs, to deployments in accessible systems. Half the population of India is not online. Layers of the stack like interfaces, devices, connectivity, languages, and costs are important to ensure access. Learning from computing fields where constraints have been embraced as design material like \textsc{ICTD} \cite{toyama2015geek} and \textsc{HCI4D} \cite{dray2012human} can help, \eg{}via delay-tolerant connectivity, low cost devices, text-free interfaces, intermediaries, and NGO partnerships (see \cite{brewer2005case, heimerl2013local, kumar2015mobile, medhi2006text, sambasivan2010intermediated, gandhi2007digital, vivek2018technology}). %As Berg argues, design is always an intervention, even when it tries be enabling and supportive of existing practices \cite{berg1998considerations}. Understanding existing infrastructures being used, whether they are technological, social, or material is important to knowing how interventions displace, augment, or threaten existing arrangements. 
% Contributing open datasets enables localisation and augmentation, strengthening the ecosystem. 
Data infrastructures to build localised datasets would enhance access equity (\eg\cite{lacuna, sambasivan2021cascades}).

%Closer to computing, cousins like ICTD  have long embraced the social sciences to develop research ethics, methods, and evaluation metrics for social justice interventions (\eg \cite{ictdethics}), which Fair-ML researchers can learn from. 

%TODO
\subsubsection{First-world care in deployments}\hfill\\
%Our study underscores the importance of design and implementation equity. 
Critiques were raised in our study on how neo-liberal AI followed a broader pattern of extraction from the `bottom billion' data subjects and labourers. Low costs, large and diverse populations, and policy infirmities have been cited as reasons for following double standards in India, \eg{}in non-consensual human trials and waste dumping \cite{macklin2004double} (also see \cite{mohamed2020decolonial}).  
Past disasters in India, like the fatal Union Carbide gas leak in 1984---one of the world's worst industrial accidents---point to faulty design and low quality, double standards for the `third world' \cite{Courttol47:online}.  
Similarly, unequal standards, inadequate safeguards, and dubious applications of AI in the non-West can lead to catastrophic effects (similar analogies have been made for content moderation \cite{roberts2016digital, sambasivan2019they}).
Fair-ML researchers should understand the systems into which they are embedding, engage with Indian realities and user feedback, and whether the recourse is meaningful. 

\vspace{-2mm}

\subsection{Enabling Fair-ML Ecosystems}

%We are currently facing a watershed moment for AI, with extravagant hype and pervasive applications. 
AI is increasingly perceived as a masculine, hype-filled, techno-utopian enterprise, with nations turning into AI superpowers \cite{Whoeverl94:online}. %Empirical studies are challenges to be `won', rather than methods to develop rigorous insights \cite{sculley2018winner}. 
AI is even more aspirational and consequential in non-Western nations, where it performs an `efficiency' function in distributing scarce socio-economic resources and differentiating economies.
For Fair-ML research to be impactful and sustainable, it is crucial for researchers to \textit{enable} a critically conscious Fair-ML ecosystem. 

\subsubsection{Ecosystems for accountability}\hfill\\
Bootstrapping an ecosystem made up of civil society, media, industry, judiciary, and the state is necessary for accountability in Fair-ML (recall the US FR example). Moving from ivory tower research approaches to solidarity with various stakeholders through partnerships, evidence-based policy, and policy maker education can help create a sustainable Fair-ML ecosystem based on sound empirical and ethical norms, \eg{} we should consider research with algorithmic advocacy groups like Internet Freedom Foundation \cite{iff}, that have advanced landmark changes in net neutrality and privacy. Efforts like the AI Observatory to catalogue, understand harms, and demand accountability of automated decision support systems in India are crucial first steps \cite{AIobs}. Technology journalism is a keystone of equitable automation and needs to be fostered for AI. 

\subsubsection{Critical transparency}\hfill\\
Inscrutability suppresses algorithmic fairness. Besides the role played by ecosystem-wide regulations and standards, radical transparency should be espoused and enacted by Fair-ML researchers committed to India. 
Transparency on datasets, processes, and models (\eg{}\cite{mitchell2019model,gebru2018datasheets,bender2018data}), openly discussing limitations, failure cases, and lessons learnt % can address practical limits and improve scientific excellence in Fair-ML in India. 
%It is also incumbent upon those in power %, \eg{}heads of organizations 
%to discuss Fair-ML as a flawed and evolving approach. 
%Such approaches 
can help move from the `magic pill' role of fairness as a checklist for ethical issues in India---to a more pragmatic, flawed, and evolving scientific function. 

%\subsubsection{Public algorithmic literacy}\hfill\\
%Our findings point to how several high-stakes decisions are made behind closed doors in India, with an unquestioned reliance on automation. AI is viewed as a neutral technology whereas datasets are full of proxies, hidden histories, and marked exclusions. Limited awareness of AI, let alone Fair-ML, may lead to uncritical adoption into public domains, regardless of consequences. Fair-ML researchers committed to India need even more to be involved in discussions with public decision-makers. Civil society is the bridge between user communities and policy, and by working directly with activist and grassroots on research and implementation, Fair-ML researchers can build AI capacity where it matters. Similarly, technology policy and the state should learn about AI and its workings and limitations, and inclusively involve consultations with civil society, technologists, and social scientists for high-stakes AI. 











\begin{comment}

\vspace{-2mm}
\section{Towards Fair-ML in India}
% \newline

%You only discover hidden biases many years down the line. The only thing worth doing is test for inequity and bias in the output. Find a way to test as soon as possible. Naive to expect to do this in training data itself. 

% Data, Model architectures, Social infrastructures, User behaviours, Justice systems all have an impact on fairness




 \begin{figure*}[ht!]
\includegraphics[width=\linewidth]{fairnessframework.png}
\caption{Steps towards Ethical AI in India.}
\label{fig:Indiaframework}
\end{figure*}

We find that several under-pinning assumptions of fair algorithms and the social infrastructures that have enabled fair outcomes in the West require re-examination in the Indian context (in Section~\ref{sec_findings}). We call upon Fair-ML researchers to take a liberatory stance towards India, moving from pedantic optimizations to a long march with the communities. We draw from Dr. B.R. Ambedkar's call of \textit{Dalit liberation}---of creating awareness, safeguards, upliftment work, and a struggle for social justice of Dalit communities \cite{jaffrelot2009dr}.% From Murray Bookchin's liberatory technologies, we ask, ``\textit{how can the new technology and resources be used in an ecological manner--that is, to promote the balance of nature, the full development of natural regions, and the creation of organic, humanistic communities?}''. 
We call upon Fair-ML researchers committed to India to take a holistic and engaged approach, to educate themselves about  the various social infrastructures, including technology policy, state, civil society, and communities. Like Donna Haraway, we ask of ourselves to `stay with the trouble',so we acknowledge our complicity, while maintaining that the goal is still recuperation \cite{haraway2016staying}. As Bonnie Nardi argues, it is necessary to innovate not just the technology, but also the logistical and social arrangements \cite{nardi2019design}. While we do not suggest a singular framework for a country as deeply plural, contradictory, and disadvantaged as India, we offer a few starting points for an algorithmic fairness agenda in India. 
An effective algorithmic fairness framework for India must not just operationalise technical fairness for the Indian context, but also innovate on how to enable justice within the surrounding social infrastructures, as shown in Figure~\ref{fig:Indiaframework} and detailed below. In table 1, we present a compilation of sub-groups, proxies, biases, and measurements in India.

%Fair-ML researchers should bridge distances: physical, emotional, and intellectual with contexts outside of the West by taking intentional steps to de-centre and check on knowledge systems.


% BH: Some points that have been made previously by others thatmight be worth re-iterating in an Indian context: 1) rather thanfocusing “top-down” on abstract definitions of fairness inspired byWestern philosophy and law, we should focus our energies “bottom-up” on the measurement of harmful discrimination, 2) focus on“studying up” by studying the cultures of the powerful in order tothrow light on processes of domination

\vspace{-2mm}
\subsection{Meaningful non-discrimination}
%\subsection{Equity in data and models}
We start by laying out how some of the existing algorithmic fairness evaluation approaches that could be translated to the Indian context and what open questions and challenges remain to effectively do this translation. 

\subsubsection{Data Infrastructure Considerations}\hfill\\
Data plays a critical role in measurements and mitigations of algorithmic bias, and is assumed to have a reliable correspondence with the people to whom we have moral obligations. However, as outlined in Section~\ref{sec_findings}, social, economic, and infrastructural factors defy this correspondence in India, challenging simplistic reliance on data. How should an algorithmic empowerment movement tackle this? We outline some recommendations and research questions regarding data and its uses in Indian contexts.  

%\begin{itemize}[leftmargin=*]
\textbf{Ontology and Epistemology}: At a fundamental level, what are the categories and constructs we model in our datasets, and how do we measure them in the world? As well as the situatedness of social categories such as gender (cf. \textit{Hijra}) and race \cite{hanna2020towards}, ontologies of affect (sentiment, inappropriateness, etc), taboos (\textit{Halal}, revealing clothing, etc), and social behaviours (headshakes, headwear, clothing, etc) are similarly contextual. How do we justify the ``knowing'' of social information by encoding it in data? 
   
\textbf{Data (Anti-)Solutions}: For which Indian contexts is being ``data-driven'' inconsistent with local values, goals and contexts?
When data are in fact appropriate for endemic goals (\eg{} caste membership for quotas), what form should their distributions and annotations take? Linguistically and culturally pluralistic communities should be given voices in these negotiations in ways that respect Indian norms of representation (\eg perhaps reservations).
    
\textbf{Relational Processes}: In fields such as health data, the vibrant role played by communities in providing, negotiating, collecting, and stewarding data, points to new ways of looking at data as dialogue (rather than operations). How does data gathering via personal relationships (such as community worker and sex worker) lead us to view data records as essentially relational, product of both beholder and the beheld? What are appropriate normative frameworks (\eg{} perhaps ethics of care \cite{held2006ethics}; see also \cite{asaro2019ai,zevenbergen2020}) for taking into account these interactions and social relations? 
Bringing the community and the commons into the data process can be starting point in establishing closeness to the data, while respecting the situated knowledge of data collectors. Multi-method understanding of data generation, through observational research and dataset analysis can help us understand usage practices, data misses, and misidentified users, which logs alone can miss. As discussed in Section~\ref{sec_background}, information transparency is critical in holding developers of datasets accountable, and accounts need to be made accessible in local languages (and in some cases non-written form, due to the high non-literacy rates in marginalized Indian populations). How might AI fairness research interface with grassroots infrastructure of data sourcing?

\textbf{Infidelities of Data}: Due to the challenges to completeness and representation discussed in Section~\ref{sec_findings}, we must be (even more than usual) sceptical of Indian datasets until they earn our trust.
And when data is neither replicable nor reproducible, when should we trust it? We must be prepared for data voids for which statistical extrapolations might not be valid. Should instances of the gamifications of recommendations data discussed in Section~\ref{sec_findings} be sought out, and if so what should we do with such gamed data?
%\end{itemize}

\textbf{Social Consent}: How might data consent work fairly in India? Ideas like collective consent \cite{MozillaF26:online}, data trusts \cite{Nesta}, and data coops could be considered for enhancing community agency in data engagements, while simultaneously increasing trustworthiness and reliability of data for algorithmic fairness. Data literacy workshops with communities marginalized by literacy and technological capital are a necessary step towards meaningful inclusion into AI, especially as beneficiaries of algorithmic fairness. %Privacy, consent, and abuse controls in AI systems should be accessible and comprehensible to marginalized communities, in their languages, cultural logics, and oppression
Can informed consent be transitive to AI if data are provided to frontline workers, built upon personal relationships and hard-earned trust?

\subsubsection{Fairness optimizations} \hfill\\
\textbf{Axes of Discrimination}: Based on a synthesis of our interviews and through desk research, we compiled a set of prominent axes along which historical injustices manifest in India, shown in Table~\ref{tab_subgroups}. 
% The table briefly summarizes how certain subgroups within each axis are historically disadvantaged and the common harms and biases that they face w.r.t. algorithmic interventions. 
% \item \textbf{Proxies and Attributes}: 
The table lists the subgroups within each axis that are historically disadvantaged, as well as some social attributes or proxies that may enable certain fairness approaches.
% Applied fairness work in the West often relies on proxy variables to approximate subgroup membership (e.g., first names as a proxy for gender, last name or zip code as proxy for race etc.). What proxies exist for the different subgroups mentioned above that may enable similar fairness research? We list some of the potential proxies for each subgroup in the Table~\ref{tab_subgroups}. 
It is important to note that names act as a signifier for various socio-demographic attributes in India, however there are no large datasets of Indian names (like the US Census data, or the SSA data) that are readily available for fairness evaluations. 
% \item \textbf{Manifestations of Injustice}: 
It is also important to note that the same subgroups may suffer discriminations very differently from the West. For instance, how gender disparities manifest in data in India would be significantly different from that in the US. How would an algorithm made fairer along gender based on datasets from the West be decontextualised and recontextualised for India? 
% Similarly, the impacts of such discrimination may also be different; for instance, \toadd{???}.
% continent masquerading as a country

\textbf{Mechanisms of Mitigation}: How might bias mitigation criteria, metrics, and methods derived using reservations systems look? As an illustration, compared to the US undergraduate admission process of selection from a pool of candidates, the undergraduate admissions in India is done through various joint seat allocation processes, over hundreds of programs, across dozens of universities and colleges that takes into account test scores, ordered preference lists, as well as various affirmative action seat reservation quotas \cite{baswana2019centralized}. The quota system gives rise to the problem of matching under distributional constraints, a known problem in economics \cite{kamada2015efficient, goto2017designing, ashlagi2020assignment}, but has not received any attention within the FAccT community.

%    \textbf{Geo-cultural Variations}: \toadd{Add a point maybe that any/all of the factors mentioned above might differ across different parts of the country due to vast cultural differences between states.}
%\end{itemize}
\vspace{-2mm}
\subsection{Empowerment}
% bootstrap a fairness ecosystem from the inside out, not outside in
Model fairness can only go so far without actual participation of communities in designing inputs, fairness approaches, and outputs. In this sub-section, we discuss how Fair-ML researchers can shift to \textit{empowering} oppressed communities in their research and policy. 
%((Ej\'{e}rcito Zapatista de Liberaci\'{o}n Nacional)

\textbf{Participatory Fair-ML knowledge systems}
% participation in knowledge 
% participation in creation
% participation in research
% participation in outcomes

Secondly, rather than treating India's population as the complexity needed to train better AI \cite{India'sm28:online}, \ie{} data subjects, we need to treat Indian user communities as bearers of their own sophisticated knowledge \cite{freire1996pedagogy} on whether, what, and how AI systems should function. Answers may lie in participatory design, a movement originating from Scandinavia in the 1970's, with deep political commitment towards democracy by siding with workers to enable change \cite{gregory2003scandinavian}. Approaches like participatory AI \cite{mitchell2016empirical}, community-based system dynamics \cite{martin2020extending}, human-centred algorithm design \cite{baumer2017toward}, and speculative design \cite{dunne2013speculative} are promising methods to identify problems and co-design responses by the communities themselves. Acknowledging differences, power distances, and shared commitments are key, as conventionally researchers have intellectual capital and assume various privileges, whereas communities we hope to serve tend to be vulnerable. Learning from decades of empirical and theoretical reflection from fields like anthropology, development studies, economics, and geography on value and methodological commitments can help. Participatory initiatives like Design Beku\footnote{https://designbeku.in/} and ? are good examples of Indic decolonial design. Pluriverses of values in algorithmic fairness in India can come from justice systems of indigenous Adivasis \cite{xaxa2011tribes}, \textit{dharma} ((social ethic) and \textit{karma} (action) from the Hindu faith,\footnote{Hindu concepts may be rejected by non-Hindus or Dalits, who see Hinduism's natural hierarchy as the contributor of the oppressive condition \cite{narayanan2001water}.}, or communism without dictatorship (\textit{sanghas}) espoused by Dr. B.R. Ambedkar, for example. 

%To audit whether outcomes are fair at the community level, looking to existing social infrastructures in India can help.  Local data officers can bridge grassroots inputs with data decision makers. How can we learn to work with existing community-led monitoring mechanisms? 

 %How can these value systems be reflected in epistemology? 
%A pluriverse of the algorithmic fairness should be broader than the normative Eurocentric knowledge of the world, made up of struggles and transformative fairness going on in the world, whether it be Ubuntu \cite{mhlambi}, Afrofuturism \cite{eshun2003further}, Pachamama \cite{tola2018between} or other non-dominant forms of knowledge. 
%However, Indic representation is not an `out there' issue for only Indians to deal with; technology makers are not impervious to biases, as evidenced in the recent caste-based oppression in Silicon Valley \cite{TheCisco63:online}. Perhaps 

%TODO
\textbf{Embrace diverse literacies and infrastructures} \hfill\\
India's heterogeneous literacies, economics, and infrastructures mean that Fair-ML researchers need to ensure that their commitment goes beyond model inferences into systems used by people. Half the population of India lacks Internet-enabled devices. Layers of the stack like user interfaces, devices, connectivity, languages, maintenance, and costs are important to consider in ensuring sustainable access and usage. Looking to the embrace of resource constraints in computing fields like \textsc{ICTD} \cite{toyama2015geek} and sub-fields of \textsc{HCI} \cite{dray2012human} can help---where constraints have been embraced as design material, in the form of technological features like delay-tolerant connectivity, low-cost devices, accessible user interfaces; partnership with civil society; and paths to sustainability like open-sourcing and capacity building \cite{brewer2005case}. As Berg argues, design is always an intervention, even when it tries to design to be enabling and supportive of existing practices \cite{berg1998considerations}. 
%Understanding existing infrastructures being used, whether they are technological, social, or material is important to knowing how interventions displace, augment, or threaten existing arrangements. 

%Closer to computing, cousins like ICTD  have long embraced the social sciences to develop research ethics, methods, and evaluation metrics for social justice interventions (\eg \cite{ictdethics}), which Fair-ML researchers can learn from. 

%TODO
\textbf{Anti-dumping stance in AI}
Critiques were raised in our study on how, similar to all other capitalistic technologies that preceded it, neo-liberal AI follows a broader pattern of extraction from `bottom billion' data subjects and AI labourers. We make an analogy here with plastic: invented as a wonder technology 1907, industry and research innovation led to applications for plastic in every sphere of human lives. Ultimately, growth of single-use plastics has led to dumping of waste in non-Western countries, causing disease, floods, and deaths (not to mention the adverse ecological impacts) \cite{PlasticP83:online}. We draw a connection to how overgrowth of AI capital, with unequal standards for non-Western countries, inadequate safeguards, and dubious applications can lead to similar catastrophic effects for the non-West, in particular. Our study underscores the importance of design and implementation equity. Past disasters in India, like the fatal Union Carbide gas leak in 1984 point to faulty design and low quality standards for `developing' countries \cite{Courttol47:online}---present day AI in India is a similar picture of poor privacy safeguards, poor pay, work, and recourse. Fair-ML researchers committed to India need to understand the systems into which they are embedding, time to respond and engage with Indian realities and user feedback, and whether the redressal is meaningful. A focus on ``studying up'' by studying the cultures of the powerful in order to throw light on processes of domination can help. 

\vspace{-2mm}
% \subsection{Debate}
\subsection{Openness}
We are currently facing a watershed moment for AI, with extravagant hype and pervasive applications. AI is increasingly imagined as a masculine, techno-utopian, and power-hungry enterprise, with nations being turned into AI superpowers and rulers of the world \cite{Whoeverl94:online}. Empirical studies are described as challenges to be `won', rather methods to develop insight \cite{sculley2018winner}. AI technologies are even more consequential and productive for postcolonial nations, where they perform a crucial `efficiency' function in distributing scarce resources, producing socio-economic benefit, and differentiating the national economy. As we see in our findings, the aspirational algorithmic imaginary in India involves visions of the fantastical, the spectacular, and unquestioned power. It is crucial for Fair-ML researchers committed to India to become attuned to broader social infrastructures, and embrace openness and public debate. 

\textbf{Openness}
Inscrutability and authority are countervailing forces for algorithmic fairness. AI/AI systems tend to be largely open-sourced and openly discussed; there is little intrinsic control that researchers have when techniques, models, and datasets are appropriated in unexpected downstream uses. Besides the role played by ecosystem-wide regulations and standards, radical openness as a design principle should be espoused and enacted by Fair-ML researchers committed to India. Disclosure of datasets, process, and inferences in publications can help. Most importantly, openly discussing limitations, failure cases, and when \textit{not} to use algorithmic fairness can help bolster the practical limits to applying computing to human problems. It is especially incumbent upon those in power, \eg{}heads of organizations and sub-organizations to discuss algorithmic fairness as an emerging, flawed, and rigorous approach. Such approaches can help mitigate the `magic pill'-role of algorithmic fairness---the solution to all neoliberal AI disparities, from hiring to datasets to knowledge, now used worldwide---to move to a pragmatic understanding of Fair-ML systems. 

\textbf{Grassroots partnerships}
Bootstrapping an ecosystem made up of civil society, media, research, industry, judiciary, and the state is necessary for Fair-ML to identify the right problems, apply scientific techniques, and ensure equitable outcomes for all sections of society. Moving from ivory tower research approaches to solidarity with various stakeholders, through project partnerships, involvement in evidence-based policy, and public education can help create a sustainable Fair-ML ecosystem based on sound empirical and theoretical basis. For example, we need to increase research collaboration with algorithmic advocacy groups Internet Freedom Foundation,\footnote{https://internetfreedom.in/} that have already advanced landmark changes in net neutrality, privacy, and surveillance. Investigative journalism on algorithms is lacking in India, but sustainable partnerships can possibly be created with people-first media sources. Algorithmic fairness and AI ethics are not mainstream research topics in Indian academia today, but academia has a pivotal role to play in advancing awareness of fairness in India, and needs funding grants for responsible AI research. A concerted effort is required from technology policy to create APIs, documentation, and voluntary open datasets in socio-economic domains. 

\textbf{Public algorithmic literacy}
Our findings point to how several high-stakes decisions are made behind closed doors in India, with an unquestioned reliance on automation. AI is viewed as a neutral technology whereas datasets are full of proxies, hidden histories, and marked exclusions. Limited awareness of AI, let alone Fair-ML, may lead to uncritical adoption into public domains, regardless of consequences. Fair-ML researchers committed to India need even more to be involved in discussions with public decision-makers. 
Civil society is the bridge between user communities and policy, and by working directly with activist and grassroots on research and implementation, Fair-ML researchers can build AI capacity where it matters. Similarly, technology policy and the state should learn about AI and its workings and limitations, and inclusively involve consultations with civil society, technologists, and social scientists for high-stakes AI. 

%whose interests does it serve, how can it challenge rather than reinforce existing sources of power, and most importantly, how its resources and attention can be marshaled to support alternative social and economic arrangements, and to help us develop a shared context and vision for the future at various scales.


\end{comment}

==> ML Fairness India Arxiv 2/findings.tex <==
 \vspace{-2mm}
\section{Findings}
\label{sec_findings}

We now present three themes (see Figure~\ref{fig:Indiadistance}) that we found to contrast views in conventional algorithmic fairness.
% In this section, we present four socio-technical infrastructures in India, that appear to contrast held views in conventional algorithmic fairness. 
%We start off with data and model considerations; followed by harms, proxies, and stereotypes faced by oppressed communities; the distance from AI researchers and makers that affects recourse and design; and AI aspirations as a developing country. 



\vspace{-2mm}
\subsection{Data and model distortions}
Datasets are often seen as reliable representations of populations.
%(based on patterns of device ownership) and phenomena.
Biases in models are frequently attributed to biased datasets, presupposing the possibility of achieving fairness by ``fixing'' the data \cite{holstein2019improving}. However, social contracts, informal infrastructures, and population scale in India lead us to question the reliability of datasets. 

 \vspace{-.5em}
\subsubsection{Data considerations} \hfill\\
\textbf{Missing data and humans}
Our respondents discussed how data points were often missing because of social infrastructures and systemic disparities in India. Entire communities may be missing or misrepresented in datasets, exacerbated by digital divides, leading to wrong conclusions \cite{barocas2016big, lerman2013big, crawford2013hidden, crawford2013think} and residual unfairness \cite{kallus2018residual}. Half the Indian population lacks access to the Internet---the excluded half is primarily women, rural communities, and Adivasis \cite{women2020mobile, InIndiaA10:online, Jain2016Indias, MissionC54:online, COVID19l97:online}. Datasets derived from Internet connectivity will exclude a significant population, \eg many argued that India's mandatory \textsc{covid}-19 contact tracing app excluded hundreds of millions due to access constraints, pointing to the futility of digital nation-wide tracing (also see \cite{AarogyaS88:online}). 
Moreover, India's data footprint is relatively new, being a recent entrant to 4G mobile data.
%Lack of digital traces may also result from poor connectivity and the abundance of informal communication (\eg{} using phone calls instead of apps) in India. 
Many respondents observed a bias towards upper-middle class problems, data, and deployments due to easier data access and revenue, as P8, CS/IS (computer science/information sciences researcher) put it, ``\textit{rich people problems like cardiac disease and cancer, not poor people's Tuberculosis, prioritised in AI [in India]}'', exacerbating inequities among those who benefit from AI and those who do not. 

\begin{figure}[t!]
\includegraphics[width=\linewidth]{fairnessdistance.png}
\caption{\small Algorithmic powerful  in India, where the distance between models and oppressed communities is large}
\label{fig:Indiadistance}
 \Description{Three screens are shown in between communities and ML models. The screens are government and civil society for AI aspiration, technology industry for third world ML treatment, and ML research for flawed data and model assumptions. The screens limit the impact of models and create distance with communities.}
\end{figure}

Several respondents pointed to missing data due to class, gender, and caste inequities in accessing and creating online content, \eg{}many safety apps use data mapping to mark areas as unsafe, in order to calculate an area-wide safety score for use by law enforcement \cite{safetipin,citizencop} (women's safety is a pressing issue in India, in public consciousness since the 2012 Nirbhaya gang rape \cite{5inNewDe60:online}. P4 (anti-caste, communications researcher) described how rape is socially (caste, culture, and religion) contextualised and some incidents get more visibility than others, in turn becoming data, in turn getting fed into safety apps---a perpetual source of unfairness. Many respondents were concerned that the safety apps were populated by middle-class users and tended to mark Dalit, Muslim, and slum areas as unsafe, potentially leading to hyper-patrolling in these areas. 

Data was reported to be `missing' due to artful user practices to manipulate algorithms, motivated by privacy, abuse, and reputation concerns. \eg{}studies have shown how women users have `confused' algorithms, motivated by privacy needs \cite{sambasivan2018privacy, masika2015negotiating}). Another class of user practices that happened outside of applications led to `off data' traces. As an example, P17, CS/IS researcher, pointed to how auto rickshaw drivers created practices outside of ride-sharing apps, like calling passengers to verify landmarks (as Indian addresses are harder to specify \cite{Economic79:online}) or cancelling rides in-app (which used mobile payments) to carry out rides for a cash payment. Respondents described how data, like inferred gender, lacking an understanding of context was prone to inaccurate inferences.

Many respondents pointed to the frequent unavailability of socio-economic and demographic datasets at national, state, and municipal levels for public fairness research. Some respondents reported on how the state and industry apparati collected and retained valuable, large-scale data, but the datasets were not always made publicly available due to infrastructure and non-transparency issues. As P5, public policy researcher, described, ``\textit{The country has the ability to collect large amounts of data, but there is no access to it, and not in a machine-readable format.''} In particular, respondents shared how datasets featuring migration, incarceration, employment, or education, by sub-groups, were unavailable to the public. Scholarship like Bond's caste report \cite{bondcaste} argues that there is limited political will to collect and share socio-economic indicators by caste or religion. 
%As another example, P22 pointed to how the 2011 Census of India data on migration was still not publicly available. 
%Many respondents discussed how institutional motivation was lacking in sharing socio-economic datasets, with high-stakes data being seen as a competitive advantage, unclear accountability for releasing datasets, and limited digitization of various public administration services. 

A rich human infrastructure \cite{sambasivan2010human} from India's public service delivery, \eg{}frontline data workers, call-center operators, and administrative staff extends into AI data collection. However, they face disproportionate work burden, sometimes leading to data collection errors \cite{datalabelling, Counting37:online, ismail2018engaging}. Many discussed how consent to a data worker stemmed from high interpersonal trust and holding them in high respect---relationships which may not be transitive to the downstream AI applications. In some cases, though, data workers have been shown to fudge data without actual conversations with affected people; efforts like \emph{jun sanwais} (public hearings) and Janata Information Systems organized by the Mazdoor Kisan Shakti Sangatan are examples to secure representation through data. \cite{singh2018, jenkins1999accounts}.
%Respondents pointed to not just the Indian datasets, but also how large and well-annotated AI datasets were lacking in non-West representation, \eg{}in Imagenet. 

\textbf{Mis-recorded identities}
Statistical fairness makes a critical assumption so pervasively that it is rarely even stated: that user data corresponds one-to-one to people.\footnote{This issue is somewhat related to what \cite{olteanu2019social} call ``Non-individual agents''.} However the one-to-one correspondence in datasets often fails in India. Ground truth on full names, location, contact details, biometrics, and their usage patterns can be unstable, especially for marginalised groups. User identity can be mis-recorded by the data collection instrument, assuming a static individual correspondence or expected behaviour. % As P24 explained, ``\textit{from a gendered perspective, women use phones less. Trying to collect data on mobile phone, you just won’t get it [...] [This] Ability to make the connection and its impact on AI is a non-trivial connection.}'' 
Since conventional gender roles in Indian society lead to men having better access to devices, documentation, and mobility (see \cite{sambasivan2018privacy, donner2008express}), women often borrowed phones. A few respondents pointed to how household dynamics impacted data collection, especially when using the door-to-door data collection method, \eg how heads of households, typically men, often answered data-gathering surveys on behalf of women, but responses were recorded as women's. 

Several AI-based applications use phone numbers as a proxy for identity in account creation (and content sharing) in the non-West, where mobile-first usage is common and e-mail is not \cite{donner2015after}. However, this approach fails due to device sharing patterns \cite{sambasivan2018privacy}, increased use of multiple SIM cards, and the frequency with which people change their numbers. Several respondents mentioned how location may not be permanent or tethered to a home, \eg{}migrant workers regularly travel across porous nation-state boundaries.

%\textbf{Non-availability and poor quality socio-economic data}

%\cite{ismail2018engaging}. However, many in our study pointed to how poor training and overburdening of data workers led to poor quality socio-economic datasets. Many respondents expressed a desire to bring communities into the data process through social audits and data trusts (\eg{}\cite{vivek2018technology}).
%Algorithmic fairness typically assumes trustworthy data handlers (for an exception, see \cite{kairouz2019advances}). However, India is considered one of the least cyber securecountries worldwide \cite{Notoriou55:online}. \eg{}Aadhaar data (identity numbers) of a billion people was available for less than 10 USD on social media \cite{Rs50010m11}. Poor privacy and security enforcement leads to a failure of the `trustworthiness' assumption by default. %Moreover, consent to a data steward, like a health worker or medical doctor, stems from high levels of trust from decades of close-knit interactions with the community, and holding such figures in high authority or respect. However, many respondents pointed to how consent may not be transitive to the usage of the data by an AI application in the downstream, particularly problematic when sought from non-literate and economically poor communities. Relatedly, P21 pointed to how dataset usage was not subject to ethical review. 
% shifting views and rewards towards accuracy of Indian data being digitized in India, e.g. acknowledging the power and implications of where this data may go, esp in healthcare, also in Aadhaar 

% TODO TODO TODO
%\vspace{-2mm}
%\subsection{Harms faced by oppressed communities}
\input{subgroups_table}
% harms to different communities
% devices and infrastructures

%TODO

\textbf{Discriminated sub-groups and proxies}
AI systems in India remain under-analysed for biases, mirroring the limited public discourse on oppression. In Table 1, we present a summary of discriminated sub-groups in India, derived from our interviews and enriched through secondary research and statistics from authoritative sources, to substantiate attributes and proxies. Furthermore, we describe below some common discriminatory proxies and attributes that came up during our interviews. While the proxies may be similar to those in the West, the implementation and cultural logics may vary in India, \eg{}P19, STS researcher, pointed to how Hijra community members (a marginalised intersex or transgender community) may live together in one housing unit and be seen as fraudulent or invisible to models using family units. Proxies may not generalise even within the country, \eg{}asset ownership: ``\textit{If you live in Mumbai, having a motorbike is a nuisance. If rural, you're the richest in town.}'' (P9, CS/IS researcher).

\begin{comment}
AI systems in India remain under-analysed for biases, mirroring the limited public discourse on oppression. Researchers have pointed to how only a minority of the privileged in India take issue with caste, religion, or ability; \eg{}in contrast to how a significant majority of white Americans oppose injustices against blacks \cite{GeorgeFl75:online}. %Oppression in India may arise from historical subordination, postcolonial poverty, and contemporary neo-liberal growth. 
In Table 1, we present a summary of axes of un-fairness in India, derived from interviews and enriched through secondary research and statistics from authoritative sources, to substantiate attributes and proxies.

%Is applying for a mobile phone or loan, and Aadhar DB being combined with other consumer DBs, and sometimes used to create private DBs. Users giving consent because they believe it will benefit them, but not understanding the power of the data they are handing off.Exclusion through 1. Recourse / explainability - not built with these users in mind 2. Tech companies "build fast and break things" mindset There were some good quotes around Indian start-ups (in FinTech I believe) on this

%\textbf{Discriminatory proxies and attributes}
%Many respondents reported that AI builders had turned a blind eye to assessing algorithms by caste, religion, and gender that AI-based discrimination was rampant and invisible. %\eg{}P4 described discrimination by caste in matimonial apps; caste was carefully considered in India's arranged marriage alliances, ``\textit{very recently a matrimonial app was accused of building a caste-based algorithm [...] If I upload my profile and say I’m a Brahmin, the algorithm detects and will not show any non-Brahmin bride to me.}'' 
Below, we describe some common, non-exhaustive discriminatory proxies and attributes to avoid, from our interviews. While the proxies may be similar to those in the West, the implementation and cultural logics may vary in India, \eg{}P19, STS researcher, pointed to how Hijra community members (a marginalised intersex or transgender community) may live together in one housing unit and be seen as fraudulent or invisible to models using family units. Proxies may not generalise even within the diverse country, \eg{}asset ownership like owning a motorbike, ``\textit{If you live in Mumbai, having a motorbike is a nuisance. If rural, you're the richest in town.}'' (P9, CS/IS researcher).
\end{comment}

\begin{itemize}[leftmargin=*]
    \item \textit{Names:} are revelatory proxies for caste, religion, gender, and ethnicity, and have contributed to discrimination in India \cite{thorat2007legacy, ChutiaCh43:online}, \eg{}Banerjee or Khan connote to caste or religion location. 
    \item \textit{Zip codes:} can correspond to caste, religion, ethnicity, or class. Many Indian zip codes are heterogeneous, with slums and posh houses abutting in the same area \cite{appadurai2000spectral,bharathi2018isolated}, unlike the rather homogeneous zip codes in the West from the segregated past \cite{ZIPCodeH5:online}.
    % (often from redlining) % and where redlining by zipcode is permissible 
    %  \cite{ZIPCodeH5:online}.
    \item \textit{Occupation:} traditional occupations may correspond to caste, gender, or religion; \eg{}manual scavenging or butchery. 
    \item \textit{Expenditure:} on dietary and lifestyle items may be proxies for religion, caste, or ethnicity; \eg{}expenses on pork or beef. 
    \item \textit{Skin tone:} may indicate caste, ethnicity, and class; however, unlike correlations between race and skin tone, correspondences to Indian sub-groups is weaker. Dark skin tones can be discriminated against in India \cite{FairButN13:online}. Many respondents described how datasets under-collected darker skin tones and measurement scales like Fitzpatrick scale are 
   not calibrated on diverse Indian skin tones.% An artefact of European colonization, light skin tones (`fair skin') is valourised in India to the point of stigmatizing darker skin tones in job applications, marriage alliances, and societal discrimination \cite{FairButN13:online} (a phenomenon common to postcolonial Africa and Asia \cite{Skinblea30:online}).
    \item \textit{Mobility:} can correlate to gender and disability. Indian women travel shorter distances and depend on public transport, for safety and cost \cite{WhyUrban26:online}. Persons with disabilities often have lower mobility in India, due to a lack of ramps and accessible infrastructure %, depending on the help of family members and passers by for mobility 
    \cite{Disabili59:online}.
    \item \textit{Language:} Language can correspond to religion, class, ethnicity, and caste. Many AI systems serve in English, which only 10\% of Indians understand \cite{InIndiaw91:online}. India has 30 languages with over a million speakers. Everyday slurs such as `dhobi', `kameena', `pariah', or `junglee' are reported to be rampant online \cite{Casteist69:online, ChutiaCh43:online}.
    \item \textit{Devices and infrastructure:} Internet access corresponds to gender, caste, and class, with 67\% Internet users being males \cite{Highgend58:online}. 
    \item \textit{Documentation}: Several AI applications require state-issued documentation like Aadhaar or birth certificates, \eg{}in finance. The economically poor are also reported to be document-poor \cite{Indiasp84:online}.\footnote{National IDs are contested in the non-West, where they are used to deliver welfare in an `objective' manner, but lead to populations falling through the cracks (see research on IDs in Aadhaar \cite{Howaglit16:online, singh2017margins}, post-apartheid South Africa \cite{donovan2015biometric} and Sri Lankan Tamils and C\^{o}te d'Ivoirians \cite{Womenand71:online}). Documentation has been known to be a weapon to dominate the non-literate in postcolonial societies \cite{gupta2012red} Also see administrative violence \cite{spade2015normal}.} 
\end{itemize}
% \vspace{-.5em}
\subsubsection{Model considerations} \hfill\\
\textbf{Over-fitting models to the privileged}
%
Respondents described how AI models in India overfitted to `good' data profiles of the digitally-rich, privileged communities, as a result of poor cultural understanding and exclusion on part of AI makers. Respondents noted that the sub-groups that had access to underlying variables for data-rich profiles, like money, mobility, and literacy, were typically middle-class men. %While the issue of model bias against minorities has been widely discussed in the West (\eg{}\cite{Aboutthe73:online}), 
Model inputs in India appear to be disproportionately skewed due to large disparities in digital access. For instance, P11, tech policy researcher, illustrated how lending apps instantly determined creditworthiness through alternative credit histories built based on the user's SMS messages, calls, and social networks (due to limited credit or banking history). Popular lending apps equate `good credit' with whether the user called their parents daily, had stored over 58 contacts, played car-racing games, and could repay in 30 days \cite{Mobilelo46:online}. Many respondents described how lending models imagined middle-class men as end-users---even with many microfinance studies showing that women have high loan repayment rates \cite{d2011women, swain2009does}. In some cases, those with `poor' data profiles subverted model predictions---as in P23's (STS researcher) research on financial lending, where women overwhelmingly availed and paid back loans in the names of male relatives to avoid perceived gender bias in credit scoring. Model re-training left new room for bias, though, due to a lack of Fair-ML standards for India, \eg{}an FR service used by police stations in eight Indian states retrained a western FR model on photos of Bollywood and regional film stars to mitigate the bias \cite{FacialRecIndia}---but Indian film stars are overwhelmingly fair-skinned, conventionally attractive, and able-bodied \cite{karan2008obsessions}, not fully representative of the larger society. 


%With over 80\% of India employed in the informal sector, running tutoring or tailoring businesses at home, \eg{}were reported to not be recorded as formal businesses, with implications for credit assessment, as P3 described, ``\textit{In a month, private tutors here can make easily 50K+ INR. He does not have a permanent job, is not in a very well known business, but still has an income level you would not be able to disambiguate from my income level.}''

%\textbf{Model provenance and portability}
%As a recent entrant to AI/AI, India was reported to import several models from the US and China. However, respondents discussed how these models were trained on non-generalizable regional datasets. Portable AI models in high-stakes domains, like crime, health, or financial risk assessment were particularly concerning due to the opacity of both training data and model behaviour \cite{mitchell2019model}. A fair model in the United States may not be fair to Indian communities. P3 pointed out ``\textit{the tool may be fair to black and white communities, but that is meaningless to Indian markets}.'' Model re-training was noted to leave new room for bias, due to a lack of standards for fairness to Indian sub-groups. \eg{}a FR service used by police stations in eight Indian states retrained a western FR model on photos of celebrities from Bollywood and other regional film industries, in order to mitigate the bias \cite{FacialRecIndia}. However, celebrities in India are overwhelmingly fair-skinned, conventionally attractive, and able-bodied \cite{karan2008obsessions}, and are not representative of the larger Indian society. 

\textbf{Indic justice in models}
Popular fairness techniques, such as equal opportunity and equal odds, stem from epistemological and legal systems of the US (\eg{}\cite{dobbe2018broader, xiang2019legal}). India's own justice approaches present new and relevant ways to operationalise algorithmic fairness locally. Nearly all respondents discussed reservations as a technique for algorithmic fairness in India. One of the restorative justice measures to repair centuries of subordination---reservations are a type of affirmative action enshrined in the Indian constitution \cite{RichardsonFairness}. Reservations assigns quotas for marginalised communities at the national and state levels.\footnote{While the US Supreme court has banned various quotas \cite{joshi2018racial}, there is a history of quotas in the US, sometimes discriminatory, \eg{New Deal black worker quotas \cite{newdeal} and anti-semitic quotas in universities \cite{hollinger1998science}}. Quotas in India are legal and common. Thanks to Martin Wattenberg for this point.} Originally designed for Dalits and Adivasis, reservations have expanded to include other backward castes, women, persons with disabilities, and religious minorities. Depending on the policy, reservations can allocate quotas from 30\% to 80\%. %Reservations are implemented in political representation, education, employment, sports, and other societal facets. 
Reservations in India have been described as one of the world's most radical policies \cite{baker_2001} (see \cite{RichardsonFairness} for more). Several studies have pointed to the successful redistribution of resources towards oppressed sub-groups, through reservations \cite{pande2003can, duflo2005political, borooah2007effectiveness}. 

%in politics, education, and employment

 \vspace{-2mm}
\subsection{Double standards by ML makers}
% Our study underscores the importance of design and implementation equity. Critiques were raised in our study on how neo-liberal AI followed a broader pattern of extraction from the `bottom billion' data subjects and AI labourers. %India, and more broadly the non-West, has been privy to unfair standards like fauly design 
%Low costs, large and diverse populations, and policy infirmities have been cited as reasons for following double standards in India, \eg{}in non-consensual human trials and waste dumping \cite{macklin2004double} (also see \cite{mohamed2020decolonial}).  
%Past disasters in India, like the fatal Union Carbide gas leak in 1984---one of the world's worst industrial accidents---point to faulty design and low quality standards for the `third world' \cite{Courttol47:online}.  %Double standards for `, research innovation on wonder technologies like plastic led to applications for plastic in every sphere of human lives, but single-use plastic overgrowth has led to dumping of waste in non-Western countries, causing disease, floods, and deaths (not to mention the adverse ecological impacts) \cite{PlasticP83:online}. 
%Similarly, overgrowth of AI capital, with unequal standards, inadequate safeguards, and dubious applications in the non-West can lead to catastrophic effects (similar analogies have been made for content moderation \cite{roberts2016digital, sambasivan2019they}).  %---present day AI in India paints a similar picture. 
%Fair-ML researchers should understand the systems into which they are embedding, respond and engage with Indian realities and user feedback, and whether the recourse is meaningful. %For example, by focus on ``studying up'' by studying the cultures of the powerful in order to throw light on processes of domination can help. 

\textbf{'Bottom billion' petri dishes}
Several respondents discussed how AI developers, both regional and international---private and state---treated Indian user communities as `petri dishes' for models. Many criticised how neo-liberal AI (including those from the state) tended to treat Indians as `bottom billion data subjects' in the periphery \cite{wallerstein1991world}---being subject to intrusive models, non-consensual automation, poor tech policies, inadequate user research, low-cost or free products that are low standard, and considered `unsaturated markets'. India's diversity of languages, scripts, and populace has been reported to be attractive for improving model robustness and training data \cite{India'sm28:online}. 
Many discussed how low quality designs, algorithms, and support were deployed for Indians, attributing to weak tech policy and enforcement of accountability in India. Several respondents described how AI makers had a transactional mindset towards Indians, seeing them as agency-less data subjects that generated large-scale behavioural traces to improve models. 

%\textbf{Poor recourse}
In contrast to how AI industry and research were moderately responsive to user bias reports in the West, recourse and redress for Indians were perceived to be non-existent. Respondents described that when recourse existed, it was often culturally-insensitive or dehumanising, \eg{}a respondent was violently questioned about their clothing by staff of a ride-sharing application, during redressal for an assault faced in a taxi (also see \cite{sambasivan2019they} for poor recourse). Several respondents described how lack of recourse was even more dire for marginalised users. \eg{}P14 (CS/IS researcher) described, ``\textit{[Ordering a ride-share] a person with a disability would choose electronic payment, but the driver insisted on cash. They said they are blind and wanted to pay electronically, but the driver declined and just moved on. No way to report it.}'' Even when feedback mechanisms were included, respondents shared that they were not always localised for India, and incidents were not always recognised unless an activist contacted the company staff directly. Many respondents shared how street-level bureaucrats, administrative offices, and front line workers---the human infrastructures \cite{sambasivan2010human} who played a crucial role in providing recourse to marginalised Indian communities---were removed in AI systems. Further, the high-tech illegibility of AI was noted to render recourse out of reach for groups marginalised by literacy, legal, and educational capital (see \cite{veeraraghavan2013dealing} for 'hiding behind a computer'). As P12 (STS researcher) explained, ``\textit{If decisions are made by a centralised server, communities don't even know what has gone wrong, why [welfare] has stopped, they don't know who to go to to fix the problem.}'' Many described how social audits and working with civil society created a better understanding and accountability.\footnote{Social audits like jan sanwais have long gauged effectiveness of civil programmes through village-level audits of documents, \eg to curb corrupt funds siphoning \cite{socialaudits}.}% for the community.%, ties with local stewards, and enabled accountability. %As P12 above said, ``\textit{How do you prove trust? One way is to have household surveys, have citizens verify, have meetings to discuss it. That's why you need a social audit.}'' 

Some respondents pointed to how Dalit and Muslim bodies were used as test subjects for AI surveillance, \eg{}pointing to how human efficiency trackers were increasingly deployed among Dalit sanitation workers in cities like Panchkula and Nagpur. Equipped with microphones, GPS, cameras, and a SIM, the trackers allowed detailed surveillance of movement and work, leading to some women workers avoiding restrooms for fear of camera capture, avoiding sensitive conversations for fear of snooping, and waiting for the tracker to die before going home \cite{Surveill67:online}. Such interventions were criticised for placing power in the hands of dominant-caste supervisors. P21 (legal researcher) pointed out that surveillance has historically been targeted at the working-poor, ``\textit{the house cleaner who is constantly suspected of stealing dried fruits or jewellery. Stepping out of their house means that their every move is tracked. Someone recording the face, the heartbeat..under the pretext of efficiency. Her job is to clean faeces in the morning and now she is a guinea pig for new AI.}'' 

\textbf{Entrenched privilege and distance}
Nearly all respondents described how AI makers and researchers, including regional makers, were heavily distant from the Indian communities they served. %Respondents had a strong perception of AI coming from American technology companies.
%(in Benjamin's words, `overserved' \cite{benjamin2019race}).
Several respondents discussed how Indian AI engineers were largely privileged class and caste males.\footnote{India fares slightly better than the US in gender representation in the tech workforce; however, gender roles and safety concerns lead to nearly 80\% of women leaving computing by their thirties (coinciding with family/parenting responsibilities) \cite{thakkar2018unexpected}.} 
For \eg{}P17 (CS/IS researcher) described, ``\textit{Who is designing AI? Incredibly entitled, Brahmin, certainly male. They've never encountered discrimination in their life. These guys are talking about primitive women. If they're designing AI, they haven't got a clue about the rest of the people. Then it becomes fairness for who?}'' Many respondents described how the Indian technology sector claimed to be `merit-based', open to anyone highly gifted in the technical sciences; but many have pointed to how merit is a function of caste privilege \cite{subramanian2015making, upadhya2007employment}. Many, though not all, graduates of Indian Institutes of Technology, founders of pioneering Indian software companies and nearly all Nobel prize winners of Indian origin have come from privileged castes and class backgrounds \cite{MostIndi27:online, subramanian2015making}. As P21 (legal researcher) explained the pervasive privilege in AI, ``\textit{Silicon Valley Brahmins [Indians] are not questioning the social structure they grew up in, and white tech workers do not understand caste to spot and mitigate obvious harms.% Identifying a white male is readily apparent across both cultures and backgrounds. Not Dalits.
}'' %Entrenched caste and religious discrimination has been documented within the tech sector \cite{Commenta9:online}, but
%Similarly, many respondents described how India was viewed as a data labour market, for annotating images and handling outsourced services, rather than for AI creation.
%is often disregarded. %As P9 (CS/IS researcher) noted, \textit{``We talk about sexuality, race, gender, but not caste. It is the white male problem of tech.''}. 
%
%As Dominant groups may wish for  western standards to continue under the pretext of merit or impartiality (goes back to critique Rawl’s merits of impartiality).
While engineers and researchers are mostly privileged everywhere, the stark socio-economic disparities between Indian engineers and the marginalised communities may further amplify the distances.

%Literature:
%stakeholders in AI: https://arxiv.org/abs/2005.07572
%https://anatomyof.AI/

 \vspace{-2mm}
\subsection{Unquestioning AI aspiration}
\textbf{AI euphoria}
Several respondents described how strong aspiration for AI for socio-economic upliftment was accompanied by high trust in automation, limited transparency, and the lack of an empowered Fair-ML ecosystem in India. Contrast with the West, where a large, active stakeholder ecosystem (of civil society, journalists, and law makers) is AI-literate and has access to open APIs and data. Many respondents described how public sector AI projects in India were viewed as modernising efforts to overcome age-old inefficiencies in resource delivery (also in \cite{sambasivan2019remarkable}). The AI embrace was attributed to follow the trajectory of recent high-tech interventions (such as Aadhaar, \textsc{MGNREGA} payments, and the National Register of Citizens \textsc{(NRC)}). Researchers have pointed to the aspirational role played by technology in India, signifying symbolic meanings of modernity and progress via technocracy \cite{pal2015banalities, pal2008computers, sambasivan2017imagined}. AI for societal benefit is a pivotal development thrust in India, with a focus on healthcare, agriculture, education, smart cities, and mobility \cite{NITI}---influencing citizen imaginaries of AI. In an international AI perceptions survey (2019), Indians ranked first in rating AI as `exciting', `futuristic' and `mostly good for society' \cite{kelley2019happy}.

Several respondents pointed to how automation solutions had fervent rhetoric; whereas in practice, accuracy and performance of systems were low. Many described how disproportionate confidence in high-tech solutions, combined with limited technology policy engagement among decision-makers, appeared to lead to sub-par high-stakes solutions, %\eg{}Delhi Police's FR service was reported to have very low accuracy \cite{fr_iff}.
\eg{}the FR service used by Delhi Police was reported to have very low accuracy and failed to distinguish between boy and girl children \cite{techcrunch}.\footnote{A confidence threshold of 80-95\% is recommended for law enforcement AI \cite{HowAccur35:online}} 
Some respondents mentioned how a few automation solutions were announced following public sentiment, but turned into surveillance \eg{}how predictive policing in Delhi and FR in train stations was announced after Nirbhaya's gruesome gangrape in 2012 and women's safety incidents \cite{Nirbhaya74:online, Facialre30:online}. %\footnote{Women's safety is a visible and pressing issue in India, and sexual assaults are widely covered by news media.}.

\textbf{Disputing AI4All}
Many respondents pointed to how emerging `4good' deployments tended to leave out minorities. \eg{}P29 (LGBTQ+ activist) discussed how AI was justified in the public domain, \eg{}surveillance for smart cities,\footnote{98 Indian cities are smart city sites, to be equipped with intelligent traffic, waste and energy management, and CCTV crime monitoring. \url{http://smartcities.gov.in/content}.} as women's safety measures, but tended to invisibilise transgender members or increase monitoring of Dalit and Muslim areas, \eg{}a FR was deployed outside women's restrooms to detect intrusion by non-female entrants, potentially leading to violence against transgender members. 

Many respondents expressed concern over AI advances in detecting sexuality, criminality, or terrorism (\eg{}\cite{seo2018partially, wang2018deep}) potentially being exported to India and harming minorities. P29 remarked on targeted attacks \cite{whatsapp}, ``\textit{part of the smart cities project is a Facial Recognition database where anyone can upload images. Imagine the vigilantism against dalit, poor, Muslims, trans persons if someone uploads a photo of them and it was used for sex offenders [arrests].}'' 


\textbf{Algorithmic opacity and authority}
In contrast to the `black box AI problem', \ie{}even the humans who design models do not always understand how variables are being combined to make inferences \cite{rudin2019we}, many respondents discussed an \textit{end-to-end} opacity of inputs, model behaviour, and outcomes in India. Fairness in India was reported to suffer from a lack of access to contributing datasets, APIs, and documentation, with several respondents describing how challenging it was for researchers and civil society to assess the high-stakes AI systems. As P11 described, ``\textit{Opacity is quite acute [in India]. People talk about blackboxes, reverse engineering inputs from outputs. What happens when you don't have the output? What happens when you can't reverse engineer at all?}''.

AI's `neutral' and `human-free' associations lent credence to its algorithmic authority. In January 2020, over a thousand protestors were arrested during protests in Delhi, aided by FR. The official statement was, ``\textit{This is a software. It does not see faith. It does not see clothes. It only sees the face and through the face the person is caught.}'' \cite{techcrunch}. While algorithms may not be trained on sub-group identification, proxies may correspond to Dalits, Adivasis, and Muslims disproportionately. \eg{}according to the National Crime Records Bureau (NCRB) in 2015, 34\% of undertrials were Dalits and Adivasis (25\% of the population); 20\% were Muslims (14\% of population); and 70\% were non-literate (26\% of the population) \cite{NCRBdata58:online}. %, similar to the black and Hispanic overrepresentation in American prisons \cite{Inaminor76:online}. 

Several respondents discussed a lack of inclusion of diverse stakeholders in decision-making processes, laws, and policies for public sector AI. Some talked about a colonial mindset of tight control in decision-making on automation laws, leading to reticent and monoscopic views by the judiciary and state. P5 (public policy researcher) pointed to how mission and vision statements for public sector AI tended to portray AI like magic, rather than contending with the realities of ``\textit{how things worked on-the-ground in a developing country}''. Additionally, respondents pointed to significant scope creep in high-stakes AI, \eg{}a few mentioned how the tender for an FR system was initially motivated by detecting criminals, later missing children, to then arresting protestors \cite{techcrunch}. 

\textbf{Questioning AI power}
Algorithmic fairness requires a buffer zone of journalists, activists, and researchers to keep AI system builders accountable. Many respondents described how limited debate and analysis of AI in India led to a weak implementation of Fair-ML in India. Issues of algorithmic bias were not widely raised in the public consciousness in India, at the time of the study. Respondents described how technology journalists in India---a keystone species for public discourse---covered app launches and investments, and less on algorithms and their impacts. P15 (journalist) pointed out that journalists may face disapproval for questioning certain narratives. \textit{``The broader issue is that AI biases do not come up in Indian press. Our definition of tech journalism has been about covering the business of tech [...] It is different from the US, where there is a more combative relationship. We don't ask tough questions of the state or tech companies.''} A seminal report by Newslaundry/Oxfam described how privileged castes comprised Indian news media, invisibilising the vast oppressed majority in public discourse \cite{Newslaundry}. %To some extent, though, verification appeared to happen at the grassroots level though methods like social audits, albeit for public welfare and not AI. %Contrast with how Propublica's pioneering investigation of risk scores for black and white defendants was aided by access to data from a public records request, jail records, race data, and the COMPAS algorithm's scores \cite{HowWeAna53:online}. (\eg{95\% of English news was written by privileged castes})




%erinarnesen: 1. There was a theme in the research about citizens feeling behind on AI advancement "Build now, let's catch up, and then let's figure out fairness."



==> ML Fairness India Arxiv 2/findings_table.tex <==

\begin{table*}
\small
%\centering
\begin{tabular}{p{1.5in}p{2in}p{2.5in}}
\toprule

\bottomrule
\end{tabular}
\normalsize
\caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
\end{table*}

==> ML Fairness India Arxiv 2/introduction.tex <==
\vspace{-2mm}
\section{Introduction}
\label{sec_intro}
%VP-META: This para says fairness research is Western and it is a bad idea

Despite the exponential growth of fairness in Machine Learning (AI) research, it remains centred on Western concerns and histories---the structural injustices (\eg{}race and gender), the data (\eg{}ImageNet), the measurement scales (\eg{}Fitzpatrick scale), the legal tenets (\eg{}equal opportunity), and the enlightenment values. Conventional western AI fairness is becoming a \textit{universal} ethical framework for AI; consider the AI strategies from India \cite{NITI}, Tunisia \cite{TunisiaAI}, Mexico \cite{MexicoAI}, and Uruguay \cite{UruguayAI} that espouse fairness and transparency, but pay less attention to what is fair in local contexts.%\footnote{By algorithmic fairness, we refer to non-discrimination towards an individual or group in AI classification.}

Conventional measurements of algorithmic fairness make several assumptions based on Western institutions and infrastructures. To illustrate, consider Facial Recognition (FR), where demonstration of AI fairness failures and stakeholder coordination have resulted in bans and moratoria in the US. Several factors led to this outcome:
\begin{itemize}[leftmargin=*]
\item Decades of scientific empiricism on proxies and scales that corresponds to subgroups in the West \cite{fitzpatrick1988validity}.
\item Public datasets, APIs, and freedom of information acts are available to researchers to analyse model outcomes \cite{MachineB33:online, HowFacia39:online}.
\item AI research/industry is fairly responsive to bias reports from users and civil society \cite{Weareimp72:online, buolamwini2018gender}.
\item The existence of government representatives glued into technology policy, shaping AI regulation and accountability  \cite{JayapalJ44:online}. 
\item An active media systematically scrutinises and reports on downstream impacts of AI systems \cite{HowFacia39:online}
\end{itemize}

%While many of these required considerable effort, 
We argue that the above assumptions may not hold in much else of the world. While algorithmic fairness keeps AI within ethical and legal boundaries in the West, there is a real danger that naive generalisation of fairness will fail to keep AI deployments in check in the non-West. Scholars have pointed to how neoliberal AI follows the technical architecture of classic colonialism through data extraction, impairing indigenous innovation, and shipping manufactured services back to the data subjects---among communities already prone to exploitation, under-development, and inequality from centuries of imperialism \cite{wallerstein1991world, kwet2019digital, mohamed2020decolonial, birhane2020algorithmic, roy2014capitalism}.
Without engagement with the conditions, values, politics, and histories of the non-West, AI fairness can be a tokenism, at best---pernicious, at worst---for communities.
If algorithmic fairness is to serve as the ethical compass of AI, it is imperative that the field recognise its own defaults, biases, and blindspots to avoid exacerbating historical harms that it purports to mitigate.
We must take pains not to develop a general theory of algorithmic fairness based on the study of Western populations.
% AI itself is exploitative to the non-West
% how can we expect fairness for one population to be equitable to all of the world?
%  Therefore, 
 %and ask---
Could fairness, then, have structurally different meanings in the non-West? Could fairness frameworks that rely on Western infrastructures be counterproductive elsewhere? How do social, economic, and infrastructural factors influence Fair-ML?

%Ultimately this is because of cultural, ethnic, and infrastructural factors, and, importantly---centuries of imperialism and neo-liberalism from the `centers' in the West have led to extraction from the `peripheries' of the non-West \cite{wallerstein1991world, Thebankt59:online, roy2014capitalism}. 


%VP-META: Now we say what we did: India (and why India)!
In this paper, we study algorithmic power in contemporary India, and holistically re-imagine algorithmic fairness in India. Home to 1.38 billion people, India is a pluralistic nation of multiple languages, religions, cultural systems, and ethnicities. India is the site of a vibrant AI workforce. Hype and promise is palpable around AI---envisioned as a force-multiplier of socio-economic benefit for a large, under-privileged population \cite{NITI}. AI deployments are prolific, including in predictive policing \cite{PredictiveIndia} and facial recognition \cite{FacialRecIndia}. 
Despite the momentum on high-stakes AI systems, currently there is a lack of substantial policy or research on advancing algorithmic fairness for such a large population interfacing with AI. %(barring the exception of \cite{marda2018artificial, marda2020data}).
% Despite the forward momentum on high-stakes AI, currently there is a lack of substantial public discourse, policy, or research on Fair-ML in India. It is important that Fair-ML community study, understand, and meaningfully advance algorithmic fairness for such a large population interfacing with AI.

We report findings from 36 interviews with researchers and activists working in the grassroots with marginalised Indian communities, and from observations of current AI deployments in India. We use feminist, decolonial, and anti-caste lenses to analyze our data. We contend that India is on a unique path to AI, characterised by pluralism, socio-economic development, technocratic nation-building, and uneven AI capital---which requires us to confront many assumptions made in algorithmic fairness. Our findings point to three factors that need attention in Fair-ML in India:

\textit{Data and model distortions}: Infrastructures and social contracts in India challenge the assumption that datasets are faithful representations of people and phenomena.  %\eg{}changing SIM cards contests one-to-one mappings of identity in data. 
Models are over-fitted for digitally-rich profiles---typically middle-class men---further excluding the 50\% without Internet access.  %\footnote{Women, rural, and Adivasi (indigenous tribes of South Asia) communities largely form the excluded half 
% \cite{InIndiaA10:online, Jain2016Indias, MissionC54:online, COVID19l97:online}. %, especially 
%women, Dalits\footnote{The caste system is a socially stratified, endogamous system of four castes, from ~1000 BC. Dalits (formerly known as `untouchables') are considered to be outside of the caste system. Dalits comprise 17\% of India's population and face heavy discrimination \cite{IndiasUn11:online}.}, Adivasis. Note: The Constitution of India refers to Dalits and Adivasis as Scheduled Castes and Scheduled Tribes respectively
Sub-groups like caste (endogamous, ranked social identities, assigned at birth \cite{ambedkar1916castes, shanmugavelan}),\footnote{According to Shanmugavelan, ``caste is an inherited identity that can determine all aspects of one’s life opportunities, including personal rights, choices, freedom, dignity, access to capital and effective political participation in caste-affected societies'' \cite{shanmugavelan}. Dalits ('broken men' in Marathi) are the most inferiorised category of the people, are within the social hierarchy, but excluded in caste categories \cite{shanmugavelan, beteille1990race, ambedkar1916castes, bondcaste}.} gender, and religion require different fairness implementations; but AI systems in India are under-analyzed for biases, mirroring the limited mainstream public discourse on oppression. Indic social justice, like reservations, presents new fairness evaluations.\footnote{We use the term 'Indic' to refer to native Indian concepts.}
%\textit{Harms and proxies of oppressed communities}: 
%AI systems in India are under-analysed for biases, mirroring the limited mainstream public discourse on oppression. 
% ; OBC (other backward classes) is a collective term used to classify other castes which are educationally or socially disadvantaged Dr. Bhimrao Ramji Ambedkar (1891–1956), fondly called Babasaheb, the uncontested leader and the dominant ideological source of Dalit politics, conceived the political category Dalit (meaning 'Broken men' in Marathi), in his attempt to reconstruct the history of untouchables in India. 

\textit{Double standards and distance by ML makers}: Indian users are perceived as `bottom billion' data subjects, petri dishes for intrusive models, and given poor recourse---thus, effectively limiting their agency.
%Recourse of marginalized Indian users,  %\footnote{We use the terms `users' and `communities' distinctly: users are AI system users; in some cases, AI might get deployed on the community, or they may lack access.} especially those dis-empowered by caste, religion, or gender, 
% are poorly addressed in AI systems built by physically and culturally distant AI makers. Indian tech workers are largely employed in low-level AI labour, with those that are in influential positions having yet to substantially contribute to India specific mitigations.
%Recourse to Indian users is anemic, indicative of a broader pattern of extraction from `bottom billion' data subjects and AI labourers is poorly addressed in AI systems. 
While Indians are part of the AI workforce, a majority work in services, and engineers do not entirely represent marginalities, limiting re-mediation of distances. 
%, within power structures of globally-unequal AI capital. A lack of meaningful redressal and safeguards has downstream implications, especially for communities marginalized by l , limiting their ability to substantially re-mediate the distances

\textit{Unquestioning AI aspiration}: 
% The AI imaginary is aspirational in India, with consequently early, and high, reliance for high-stakes domains. Limited algorithm analysis mechanisms and inclusion of stakeholders contributes to this view and implies a missing, but necessary ecosystem to implement fair inferences in communities. 
% The AI imaginary is aspirational; AI is readily adopted in high-stakes domains, often too early. Lack of an ecosystem of tools, policies, and stakeholders (\ie{} critical journalists, researchers, and lawmakers) to interrogate high-stakes AI is an impediment in ensuring meaningful fairness 
The AI imaginary is aspirational in the Indian state, media, and legislation. AI is readily adopted in high-stakes domains, often too early. Lack of an ecosystem of tools, policies, and stakeholders like journalists, researchers, and activists to interrogate high-stakes AI inhibits meaningful fairness in India.

%this aspirational and optimistic nature is in part due to a lack of adequate interrogation of these systems, 

%AI is aspirationally viewed in India,  Subsequently, there is unquestioning reliance on automation in a developing economy, with minimal checks and safeguards, a lack of questioning of algorithmic power, and inscrutability of data and inferences for civil society.%---the activation layers for fairness implementation in society. 

In summary, we find that conventional Fair-ML may be inappropriate, insufficient, or even inimical in India if it does not engage with the local structures. In a societal context where the distance between models and dis-empowered communities is large---via technical distance, social distance, ethical distance, temporal distance, and physical distance---a myopic focus on localising fair model outputs alone can backfire. 
We call upon fairness researchers working in India to engage with \emph{end-to-end} factors impacting algorithms, like datasets and models, knowledge systems, the nation-state and justice systems, AI capital, and most importantly, the oppressed communities to whom we have ethical responsibilities. We present a holistic framework to operationalise algorithmic fairness in India, calling for: \textit{re-contextualising} data and model fairness; \textit{empowering} oppressed communities by participatory action; and \textit{enabling} an ecosystem for meaningful fairness. 

Our paper contributes by bringing to light how algorithmic power works in India, through a bottom-up analysis. Second, we present a holistic research agenda as a starting point to operationalise Fair-ML in India. The concerns we raise may certainly be true of other countries. The broader goal should be to develop global approaches to Fair-ML that reflect the needs of various contexts, while acknowledging that some principles are specific to context.

%We present an opportunity to go beyond localisation of data and model fairness alone, to meaningfully impact the Indian population. 

%We demonstrate that the assumptions of algorithmic fairness do not scale neatly to India.  

==> ML Fairness India Arxiv 2/method.tex <==
\vspace{-2mm}

\section{Method}
\label{sec_methodology}
Our research results come from a critical synthesis of expert interviews and discourse analysis. Our methods were chosen in order to provide an expansive account of who is building ML for whom, what the on-the-ground experiences are, what the various processes of unfairness and exclusions are, and how they relate to social justice. 

We conducted qualitative interviews with 36 expert researchers, activists, and lawyers working closely with marginalised Indian communities at the grassroots. 
Expert interviews are a qualitative research technique used in exploratory phases, providing practical insider knowledge and surrogacy for a broader community \cite{bogner2009interviewing}. Importantly, experts helped us gain access to a nascent and difficult topic, considering the early algorithmic deployments in the public sector in India.
% Expert interviews are a qualitative research technique used in exploratory phases, providing practical insider knowledge, surrogacy for a broader community, and importantly---with the early algorithmic deployments in the public sector in India, experts helped gain access to a nascent and difficult topic \cite{bogner2009interviewing}.
Our respondents were chosen from a wide range of areas to create a holistic analysis of algorithmic power in India. Respondents came from Computer Science (11), Activism (9), Law and Public Policy (6), Science and Technology Studies (5), Development Economics (2), Sociology (2), and Journalism (1). All respondents had 10-30 years of experience working with marginalised communities or on social justice. Specific expertise areas included caste, gender, labour, disability, surveillance, privacy, health, constitutional rights, and financial inclusion. 24 respondents were based in India, 2 in Europe, 1 in Southeast Asia, the rest in the USA; 25 of them self-identified as male, 10 as female, and 1 as non-binary.

In conjunction with qualitative interviews, we conducted an analysis of various algorithmic deployments and emerging policies in India, starting from Aadhaar (2009).
We identified and analysed various Indian news publications (\eg{}TheWire.in, Times of India), policy documents (\eg{}NITI Aayog, Srikrishna Bill), and community media (\eg{}Roundtable India, Feminism in India), and prior research. Due to secondary sources, our citations are on the higher side.
% 

\textbf{Recruitment and moderation}
We recruited respondents via a combination of reaching out directly and personal contacts, using purposeful sampling \cite{palinkas2015purposeful}---\ie identifying and selecting experts with relevant experience---iterative until saturation. We conducted all interviews in English (preferred language of participants). The semi-structured interviews focused on 1) unfairness through discrimination in India; 2) technology production and consumption; 3) the historical and present role of fairness and ethics in India; 4) biases, stereotypes and proxies; 5) data; 6) laws and policy relating to fairness; and 7) canonical applications of fairness, evaluated in the Indian context. Respondents were compensated for the study (giftcards of 100 USD, 85 EUR, and 2000 INR), based on purchasing power parity and non-coercion. Employer restrictions prevented us from compensating government employees. Interviews lasted an hour each, and were conducted using video conferencing and captured via field notes and video recordings. 

\textbf{Analysis and coding}
Transcripts were coded and analyzed for patterns using an inductive approach~\cite{Thomas2006general}. From a careful reading of the transcripts, we developed categories and clustered excerpts, conveying key themes from the data. Two team members created a code book based on the themes, with seven top-level categories (sub-group discrimination, data and models, law and policy, ML biases and harms, AI applications, ML makers, and solutions) and several sub-categories (\eg{}caste, missing data, proxies, consent, algorithmic literacy, and so on). The themes that we describe in Section~\ref{sec_findings} were then developed and applied iteratively to the codes.

Our data is analysed using feminist, decolonial, and anti-caste lenses. A South Asian feminist stance allows us to examine oppressed communities as encountering and subverting forces of power, while locating in contextual specifics of family, caste, class, and religion.\footnote{We are sympathetic to Dalit feminist scholars, like Rege, who have critiqued postcolonial or subaltern feminist thoughts for the lack of anti-caste scrutiny \cite{rege1998dalit}} South Asian feminism is a critique of the white, Western feminism that saw non-western women as powerless victims that needed rescuing \cite{mohanty2005feminism, chaudhuri2004feminism}. 
Following Dr. B. R. Ambedkar's insight on how caste hierarchies and patriarchies are linked in India \cite{chakravarti1993conceptualising}, we echo that no social justice commitment in India can take place without examining caste, gender, and religion. A decolonial perspective (borrowed from Latin American and African scholars like \cite{escobar2011encountering, mignolo2011darker, wa1992decolonising,fanon2007wretched, dorfman1975read}) helps us confront inequalities from colonisation in India, providing new openings for knowledge and justice in AI fairness research. To Dr. B. R. Ambedkar and Periyar E. V. Ramasamy, colonialism predates the British era, and decolonisation is a continuum. For Dalit emancipatory politics, deconstructing colonial ideologies of the powerful, superior, and privileged begins by removing influences and privileges of dominant-caste members.\footnote{Thanks to Murali Shanmugavelan for contributing these points.}

%Recent critics from postcolonial studies reject Mignolo's 'decoloniality' – a recognition to the theorisation of separate knowledge systems and alternative epistemes. 

\textbf{Research ethics}
We took great care to create a research ethics protocol to protect respondent privacy and safety, especially due to the sensitive nature of our inquiry. During recruitment, participants were informed of the purpose of the study, the question categories, and researcher affiliations. Participants signed informed consent acknowledging their awareness of the study purpose and researcher affiliation prior to the interview. At the beginning of each interview, the moderator additionally obtained verbal consent. We stored all data in a private Google Drive folder, with access limited to our team. To protect participant identity, we deleted all personally identifiable information in research files. We redact identifiable details when quoting participants. Every respondent was given the choice of default anonymity or being included in Acknowledgements. 

%\subsection{Reflexivity}
All co-authors of this paper work at the intersection of under-served communities and technology, with backgrounds in HCI, critical algorithmic studies, and ML fairness. The first author constructed the research approach and has had grassroots commitments with marginalised Indian communities for nearly 15 years. The first and second author moderated interviews. All authors were involved in the framing, analysis, and synthesis. Three of us are Indian and two of us are White. All of us come from privileged positions of class and/or caste. We acknowledge the above are our interpretations of research ethics, which may not be universal. %The first author has 15 years of grassroots experience with technology design with marginalised communities in India. 

%The effect of the cultural bomb is to annihilate a people's belief in their names, in their languages, in their environments, in their heritage of struggle, in their unity, in their capacities and ultimately in themselves
%change will only happen when the proletariat is empowered by their own language and culture.[13]
%the rhetoric of modernity is the constant updating of the rhetoric of salvation hiding the logic of coloniality – war, destruction, racism, sexism, inequalities, injustice, etc.

%Fanon positions decolonization as chaotic, an unclean break from a colonial condition that is already over determined by the violence of the colonizer and unresolved in its possible

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> ML Fairness India Arxiv 2/subgroups_table.tex <==
\begin{savenotes}
\begin{table}
\small
%\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{\linewidth}{X}
\toprule
\multicolumn{1}{c}{\bf Sub-groups, Proxies and Harms} \\
\midrule
\begin{minipage}[t]{\linewidth}
\textbf{Caste} 
\footnotesize{(17\% Dalits; 8\% Adivasi; 40\% Other Backward Class (OBC)
% \footnote{The Constitution of India refers to Dalits and Adivasis as Scheduled Castes and Scheduled Tribes respectively; Other Backward Castes is a collective term used to classify castes which are educationally or socially disadvantaged}
)\cite{CensusIndia2011}} %\newline 
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
  \item \footnotesize{Societal harms: Human rights atrocities. Poverty. Land, knowledge and language battles  \cite{xaxa2011tribes, ambedkar2014annihilation, Twothird31:online}. }
    \item \footnotesize{Proxies: Surname. Skin tone. Occupation. Neighborhood. Language.} %\newline
    \item \footnotesize{Tech harms: Low literacy and phone ownership. Online misrepresentation \& exclusion. Accuracy gap of Facial Recognition {(FR)}. Limits of Fitzpatrick scale. Caste-based discrimination in tech ({}\cite{TheCisco63:online}). }
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule

\begin{minipage}[t]{\linewidth}
\textbf{Gender}
\footnotesize{(48.5\% female)\cite{IndiaMinistryStatistics2018}} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Sexual crimes. Dowry. Violence. Female infanticide.}
  \item \footnotesize{Proxies: Name. Type of labor. Mobility from home. }%
    \item \footnotesize{Tech harms: Accuracy gap in FR. Lower creditworthiness score. Recommendation algorithms favoring majority male users. Online abuse and 'racey’ content issues. Low Internet access.} 
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule

\begin{minipage}[t]{\linewidth}
\textbf{Religion}
\footnotesize{(80\% Hindu, 14\% Muslim, 6\% Christians, Sikhs, Buddhists, Jains and indigeneous) \cite{CensusIndia2011}}  %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Discrimination, lynching, vigilantism, and gang-rape against Muslims and others \cite{84DeadIn98:online}.}
    \item \footnotesize{Proxies: Name. Neighborhood. Expenses. Work. Language. Clothing. } %\newline
    \item \footnotesize{Tech harms: Online stereotypes and hate speech, \eg Islamophobia. Discriminatory inferences due to lifestyle, location, appearance. Targeted Internet disruptions.} %%\newline}
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule

\begin{minipage}[t]{\linewidth}
\textbf{Ability}
\footnotesize{(5\%--8\%+ persons with disabilities) \cite{WorldBank2009Disabilities}} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Stigma. Inaccessible education, transport \& work.} 
    \item \footnotesize{Proxies: Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices.} %\newline
    \item \footnotesize{Tech harms: Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. }%\newline
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule


\begin{minipage}[t]{\linewidth}
\textbf{Class}
\footnotesize{(30\% live below poverty line; 48\% on \$2--\$10/day)\cite{Rangarajan2014Poverty}}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Poverty. Inadequate food, shelter, health, \& housing.}
    \item \footnotesize{Proxies: Spoken \& written language(s). Mother tongue. Literacy. Feature / Smart Phone Ownership. Rural vs. urban.}
    \item \footnotesize{Tech harms: Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access. }%\newline
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule

\begin{minipage}[t]{\linewidth}
\textbf{Gender Identity \& Sexual Orientation}
\footnotesize{(No official LGBTQ+ data)} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    % \item \footnotesize{Societal harms: Colonial law 377, but discrimination and abuse persist.} 
    \item \footnotesize{Societal harms: Discrimination and abuse. Lack of acceptance and visibility, despite the recent decriminalisation.\cite{tamang2020section}} 
    \item \footnotesize{Proxies: Gender declaration. Name. }%
    \item \footnotesize{Tech harms: FR "outing" and accuracy. Gender binary surveillance systems (\eg in dormitories). M/F ads targeting.  Catfishing and extortion abuse attacks.}
\end{itemize}
\end{minipage}\vspace{2pt}\\
\midrule

\begin{minipage}[t]{\linewidth}
\textbf{Ethnicity}
\footnotesize{(4\% NorthEast) \cite{CensusIndia2011}}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Racist slurs, discrimination, and physical attacks.}
    \item \footnotesize{Proxies: Skin tone. Facial features. Mother tongue. State. Name. }
    \item \footnotesize{Tech harms: Accuracy gap in FR. Online misrepresentation \& exclusion. Inaccurate inferences due to lifestyle, \eg migrant labor. }%\newline
\end{itemize} 
\end{minipage}\vspace{2pt}\\
\bottomrule
\end{tabularx}
\normalsize
\vspace{2pt}
\caption{\label{tab_subgroups} \small Axes of potential ML (un)fairness in India%: sub-groups, proxies, and harms.
}
\end{table}
\end{savenotes}






% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabularx}{\textwidth}{p{1.5in} X p{2in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits; 8\% Adivasi; 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female; Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim; 7\% Other; 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on \$2-\$10/day
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day; 11\% speak English; 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. Rural vs. urban.
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule

% % \begin{comment}
% % \textbf{Region}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \midrule
% % \textbf{Gender identity}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \bottomrule
% % \end{comment}

% \end{tabularx}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}








%VP: Backup before compressing

% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabular}{p{1.5in}p{2in}p{2.5in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits \newline
% \tabitem 8\% Adivasi \newline
% \tabitem 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female \newline
% \tabitem Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim \newline
% \tabitem 7\% Other \newline
% \tabitem 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule
% \begin{comment}
% \textbf{Region}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \midrule
% \textbf{Gender identity}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \bottomrule
% \end{comment}
% \end{tabular}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}



==> ML Fairness India Arxiv 2/subgroups_table2.tex <==
\begin{table}
\small
%\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{.95\linewidth}{X}
\toprule
\multicolumn{1}{c}{\bf Sub-groups, Proxies and Harms} \\
\midrule

\textbf{Caste} 
(17\% Dalits; 8\% Adivasi; 40\% Other Backward Class (OBC))\cite{CensusIndia2011} %\newline 
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
   \item \footnotesize{Societal harms: Human rights atrocities. Poverty. Land, knowledge and language battles  \cite{xaxa2011tribes, NCRBdata58:online, Twothird31:online}. }
    \item \footnotesize{Proxies: Surname. Skin tone. Occupation. Neighborhood. Language.} %\newline
    \item \footnotesize{Tech harms: Low literacy and phone ownership. Online misrepresentation \& exclusion. Accuracy gap of Facial Recognition {(FR)}. Limits of Fitzpatrick scale. Caste-based discrimination in tech {}\cite{TheCisco63:online}. }
\end{itemize}
\midrule
\textbf{Gender}
(48.5\% female)\cite{IndiaMinistryStatistics2018} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Sexual crimes. Dowry. Violence. Female infanticide.}
  \item \footnotesize{Proxies: Name. Type of labor. Mobility from home. }%
    \item \footnotesize{Tech harms: Accuracy gap in FR. Lower creditworthiness score. Recommendation algorithms favoring majority male users. Online abuse and 'racey’ content issues. Low Internet access.} 
\end{itemize}

\midrule
\textbf{Gender Identity \& Sexual Orientation}
(No official LGBTQ+ data) %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Colonial law 377 traces. Discrimination and abuse.} 
    \item \footnotesize{Proxies: Gender declaration. Name. }%
    \item \footnotesize{Tech harms: FR "outing" and accuracy. Gender binary surveillance systems in public spaces, \eg dormitories. M/F ads targeting.  Catfishing and extortion abuse attacks.}
\end{itemize}
\midrule

\textbf{Religion}
(80\% Hindu, 14\% Muslim, 6\% Christians, Sikhs, Buddhists, Jains and indigeneous) \cite{CensusIndia2011}  %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Discrimination, lynching, vigilantism, and gang-rape against Muslims and others \cite{84DeadIn98:online}.}
    \item \footnotesize{Proxies: Name. Neighborhood. Expenses. Work. Language. Clothing. } %\newline
    \item \footnotesize{Tech harms: Online stereotypes. Targeted hate speech, \eg Islamophobia. Discriminatory inferences due to lifestyle, location, appearance. Targeted Internet disruptions.} %%\newline}
\end{itemize}
\midrule

\textbf{Ability}
(5\%--8\%+ persons with disabilities) \cite{WorldBank2009Disabilities} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Stigma. Inaccessible education, transport \& work.} 
    \item \footnotesize{Proxies: Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices.} %\newline
    \item \footnotesize{Tech harms: Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. }%\newline
\end{itemize}
\midrule


\textbf{Class}
(30\% live below poverty line; 48\% on \$2--\$10/day)\cite{Rangarajan2014Poverty} \cite{CensusIndia2011}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Poverty. Inadequate food, shelter, health, \& housing.}
    \item \footnotesize{Proxies: Spoken \& written language(s). Mother tongue. Literacy. Feature/Smart Phone Ownership. Rural vs. urban.}
    \item \footnotesize{Tech harms: Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access. }%\newline
    \end{itemize}
\midrule

\textbf{Ethnicity}
(4\% NorthEast) \cite{CensusIndia2011}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Northeastern Indians face racist slurs, discrimination, and violent attacks.}
    \item \footnotesize{Proxies: Skin tone. Facial features. Mother tongue. State. Name. }
    \item \footnotesize{Tech harms: Accuracy gap in FR. Online misrepresentation \& exclusion. Inaccurate inferences due to lifestyle, \eg migrant labor. }%\newline
\end{itemize}
\bottomrule
\end{tabularx}
\normalsize
\caption{\label{tab_subgroups} Axes of potential ML (un)fairness in India: sub-groups, marginalized groups, proxies, and harms.
}
\end{table}







% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabularx}{\textwidth}{p{1.5in} X p{2in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits; 8\% Adivasi; 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female; Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim; 7\% Other; 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on \$2-\$10/day
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day; 11\% speak English; 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. Rural vs. urban.
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule

% % \begin{comment}
% % \textbf{Region}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \midrule
% % \textbf{Gender identity}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \bottomrule
% % \end{comment}

% \end{tabularx}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}








%VP: Backup before compressing

% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabular}{p{1.5in}p{2in}p{2.5in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits \newline
% \tabitem 8\% Adivasi \newline
% \tabitem 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female \newline
% \tabitem Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim \newline
% \tabitem 7\% Other \newline
% \tabitem 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule
% \begin{comment}
% \textbf{Region}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \midrule
% \textbf{Gender identity}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \bottomrule
% \end{comment}
% \end{tabular}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}



==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> changelog.tex <==
Quick Links
Internal Feedback
Interviewee Feedback
Acks

Internal Feedback

Daniel Russel
Overall, an interesting paper that I appreciate, but I feel as though I'm missing a few things. First: Where's this going? What conference do you want to submit this to? Is this an opinion piece? An overview? A featured article? What's the role that you're intending for this article?
Apologies! This is a paper submission for FaccT 2021, formerly FAT*. They have a Human Factors (HCI) track, under which we’re submitting this paper.

While I feel as though it would be a valuable article for the greater community, I think this will need to also be approved by PR before publication.
We have sought approvals from P-counsel, PR, Comms and Policy and already have an LGTM from P-counsel. We’ll update the thread once we get LGTMs from other parties.

A couple of quick comments:

* the summary seems cut off... it ends mid-sentence. Is there supposed to be more there?
In general, the paper has become a lot tighter and has more of a flow since a week ago. These formatting issues have been identified and fixed.

* the copyright notice (page 1) is strange and odd. Woodstock?
Yeah, this is the new ACM sigconf template

* the Mortimer Adler reference is fairly second hand and seems inconsistent with the paper you're trying to write. That story is reported as "the story is told of Mortimer Adler attending.." (I see your point, but that's a slim, dubuious story to base such an essential argument on.)
Thanks for pointing this out. We’ll be on the lookout for a better reference to bring out the ‘justice’ in America vs. ‘harmony’ in the East. For now we’ll scrap this reference.  

* you write that "AI/ML systems tend to be largely open-sourced and openly discussed.." (in Openness), but then write "Our findings point to how several high-stakes decisions are made behind closed doors in India.." (in Public Algorithm Literacy). I think I see what you mean, but both things probably can't be true. (And I'm not even sure that "AI/ML systems tend to be largely open-sourced..." -- there ARE a lot of open-source libraries that are available, but there is also a LOT of non-open-sourced code that's in common use. Do you know of any way to estimate the quantity of each?)
Thanks for pointing this out. The text has changed since then and now we don’t have a mention of open-sourced models. Though originally we didn’t mean it as open source code, but as openly scrutable models and outputs. But I suppose it wasn’t clear :).

* unclear to me how quoting the Zapatistas will help your argument. ("As the Zapatistas said..") The citation is missing, but I don't know how a rhetorical line from a political/miltant group will advance the story you want to tell. Since that section starts with Mbembe's critique of objectivism and goes on to argue for making inclusive knowledge production, you could probably lose that sentence and improve the readability of the section.
This was a bit challenging, as the Zapatista quote is deeply cherished in the decolonial theory circles, which originated in Latin America and saw the Zapatista movement as an indigeneous expression of autonomy. But given the militant implications you rightly point out, we have now removed the sentence. The readability is also better now, going straight to Mbembe.

* the phrase "communism without dictatorship (sanghas) espoused by Dr. B.R. Ambedkar," probably needs a citation. I'm not familiar enough with this to know what you're referring to. (Is this also from [53]?)
Thanks, added now.

* Biggest question: How did you go from your research Method ("interviewing with 36 expert researchers, activists, and lawyers working closely with marginalized Indian communities" then coding those interviews) to the Findings of Section 4? There's no description of the clustering / topic-identification process you followed to determine that these topics ("Missing data," "one-to-one correspondence," "Good data profiles," etc.) were the most important topics that emerged from the interviews with the "researchers, activists, and lawyers." What was that process?
Great point! An obvious miss on my part. New addition in Method: 
“Transcripts were coded and analyzed for patterns using an inductive approach~\cite{Thomas2006general}. From a careful reading of the transcripts, we developed categories and clustered excerpts, conveying key themes from the data. Two team members created a code book based on the themes, with seven top-level categories (sub-group discrimination, data and models, law and policy, biases, AI applications, ML makers, and solutions) and several sub-categories (\eg{}caste, missing data, proxies, consent, algorithmic literacy, and so on). The three power structures that we describe below were then developed and applied iteratively to the codes.”

For instance, in section 4.2, where did Table 1 come from? ("Axes of potential (un)fairness in India") You say that the table is "(by no means exhaustive, but representative of our interview results)." But there's a lot of numeric data there (e.g., caste population sizes)... where did THAT come from? (Later you say it's a composite of your interviews and "desk research" but you're presenting data without citation or sources.)
Thanks for pointing this out. We now have body text saying,
“In Table 1, we present a summary of axes of discrimination in India, derived from interviews and enriched through secondary research and statistics from authoritative sources, to substantiate attributes and proxies.”


Jess Holbrook

Introduction
"We contend that India is on an alternative path to AI, characterised by pluralism, socio-economic development, technocratic nation-building, and unequal AI capital—which requires us to confront many assumptions made in conventional algorithmic fairness." - may want to make explicit what this an alternative to, it is implied but may benefit from being explicit
The "ML makers’ distance:" paragraph was a bit unclear to me. I think you're trying to make two points that might be separated - 1) ML makers are both physically and culturally distant from their users and 2) even when they are close, they are at less influential points in the development pipeline and not in a position to remediate those distances.
"The AI imaginary" - do you mean imagination? 
The "AI aspiration:" paragraph seems like it has two distinct ideas in it - 1) the imagination is aspirational and a consequence is it is being used in high stakes domains, perhaps too early and 2) this aspirational and optimistic nature is in part due to a lack of adequate interrogation of these systems, which requires the right ecosystem of tools, policies, processes, etc.
Table 1
Colonial law 377 traces - I'm not familiar with this one but just might be me. Calling out that it may not be 100% clear to readers what this means.
4.2 ML makers' distance
"Many respondents shared how street-level bureau-crats, administrative offices, and front line workers—the human infrastructures who played a crucial role in providing recourse to marginalised Indian communities—were removed in ML systems." - I love insights like this. So good.
5.1.1 Data Considerations
"when data is neither replicable nor reproducible, what conditions can we set to expect reliability?" - I wasn't sure what this meant
I may have missed it but do you call for more open data sets in this section? That would go a long way with transparency and you could link it to projects like the Lacuna Fund and how these datasets can enable local developer ecosystems. It could go in 5.3 as well. 
Alex Hanna:
Thanks for this paper, Nithya and Vinod. It's really insightful and revealing. I have some general comments on this paper, and then some more specific recommendations for other references. My more general comments are that this paper is doing a lot. I think the critique of the Western-centric notions of fairness and fair-ML are all on point, and Table 1 is really helpful for this. My more specific version of the comments are mostly around Section 5, which I think points to many directions for future action, but is also very ambitious insofar as who is going to adopt these suggestions. For instance, is this targeted towards fair-ML people, or AI practitioners writ large? Is this targeted towards participatory partners? I think sharpening the imaginary audience can help prioritize which of the recommendations you'd like to dig into in deep detail. Because I'm interested most in data infrastructure, I find that I want more there, bu I think the considerations of empowerment would appeal more to design-forward scholars and practitioners, and openness perhaps to model builders.
 
More specifically, some thoughts and references which can be helpful --
 
There's some ethnographic work by STSer Ranjit Singh on Aadhaar which could be relevant here --
- https://dl.acm.org/doi/10.1145/3025453.3025910
- https://www.tandfonline.com/doi/abs/10.1080/00856401.2019.1602810?journalCode=csas20
 
There's a connection of "document poverty" to Dean Spade's idea of administrative violence and the mismatch of one's identity docs, especially for trans people.
 
"Optimization strategies in algorithmic fairness, such as equal opportunity or equal odds, stem from epistemologies and legalities of the United States."
- I'd also say they are based in a "perpetrator-based" perspective, rather than "victim-based" one, which has been critiqued by critical race scholarship (cf. Alan Freeman). The rights-based perspective has always been narrowly "white", to be blunt. Also see Dean Spade on this.
 
"In India, the strong aspiration for social and economic upliftment was also reported to be accompanied by unquestioning trust in automation and minimal checks and balances."
- Lilly Irani's book might be a good reference here: https://www.google.com/books/edition/Chasing_Innovation/tbZuDwAAQBAJ?hl=en&gbpv=1&printsec=frontcover
 
Reena:

Comments provided in-line here.

Martin
Hi Nithya,
 
Sounds like an impressive set of work, and thanks for sending that paper--very interesting! Yes, please do send the latest research agenda doc.
 
Super-dumb question on the paper: what's the difference between "Indic" and "Indian"?
 
Open-ended question: the paper describes quotas (reservations) as an Indic approach to fairness, different from the US. But the US has a long history of quota systems. Of course, some types of quotas are currently illegal, but not all of them (to give just one example, today government contracts have to go to a certain percentage of businesses owned by minorities/women/veterans). Historically, quotas have been used in the US for a long time... in the New Deal in the 30s, some agencies had to give a certain percentage of jobs to Black workers. At the same time, there were also notorious quotas that put a cap on minorities (e.g., on Jewish applicants to elite colleges, for a while, allowing no more than something like 15%). So quotas are definitely a very familiar (if controversial) technique in the US. Is the difference in India that they're always legal, and people support them without any controversy? 

--Martin



Feedback on paper from interviewees: 
Ranjit:
The last sentence of Missing data and invisible humans in Section 4.1.1 Data considerations, which focuses on trust in data workers requires more nuance. I believe the story is more complicated than placing trust in data workers. There have also been situations when data workers have entered data incorrectly without actual conversations with people affected by changes in their data records. As a result, there have been social movements in India organized by the Right to Information activists (MKSS, more specifically) on securing representation through data along with calls for Janata Information Systems. See also the attached paper. 
In the same section, when talking about Axes of un-fairness, harms, and discriminatory proxies, another issue to consider is literacy and how it constrains the ability of a person in becoming digitally-rich as already indicated in the first paragraph of Section 4.1.2 Model Considerations.
Section 4.2 ML Markers' distance ends with a discussion on developers of AI belonging to privileged castes and middle-class backgrounds, but it ends in a quote talking about "white male problem of tech". To me, it felt kind of jarring because the developers referred to in the paragraph are not typically "white." It seemed to me like a conflation of two different problems of contending with race and caste that are similar but not the same. 
Savita:
- In addition to opening up the research & policy debates, would you hope for a set of principles specific to country contexts? In doing so, is that acknowledging that some principles are not universal?
- you mention the AI imaginary is aspirational. It might be worth clarifying all the stakeholders for whom it's aspirational (you mention initiatives but are they led by any particular driver?)
- In research ethics, you talk about being careful on consent, storing documentation safely etc. You also acknowledge yourselves as privileged (a nice touch!) but is it worth making the link between the two more explicit by saying something like you acknowledge these are your interpretations of research ethics, which may also not always be universal? Don't know if that is too risky to say!
 
Aneesh:
Good to hear from you. The paper looks wonderful. I have only one citation idea, my 2006 book, Virtual Migration :-). It was the first work (apart from my 2001 dissertation) to talk about algorithmic power; it developed the whole theory of algocracy. 
 
Murali:
Thanks for the patience, and I am attaching my comments/observations. Some are more pertinent than others. I am aware that this delay is not ideal, but I hope this is still useful to authors.
Two general comments:
As happens in the race and technology domain where collaboration with black scholars is a valued as a sign of ethical and political position, I sincerely hope future discussions about building caste-sensitive include Dalit and anti-caste scholars/activists. I am confident that authors will move towards that direction in their next phase.
This exciting paper has a lot of scopes to refer to Dalit and Adivasi scholarships (e.g., feminist/poco/media-cultural critiques) and in turn, could benefit from their critical insights. After all, each citation is political.
 
Follow-up from Murali
Last week, I gave a talk on "Caste in legal regimes" at King's India Institute: I argued how "unconventional legal regimes" - on sites such as the Internet - are now replacing  "conventional legal regimes."  
 
I presented an analysis of how a western legal doctrine (the impartiality test) - despite well-meaning intentions - might enable casteism on the Internet. I have to find out if they recorded the talk and would upload it.
 
A succinct discussion on the manifestation of "modern caste" (and other relevant non-western categories) and its everyday communicative practice is very relevant to the scope of the paper.
 
As you well know, I am very keen to be part of any future discussions on this topic.Thank you.
Attachments - Bond Caste & Development; Caste Definitions
Best wishes,
Murali
 
PS: do see our arguments related to caste and (lack of) disaggregated data in BOND Caste and Development Report
 
(350 words allowed)
Thanks to the reviewers for their valuable comments. We believe our paper makes a critical contribution to shift the boundaries of the current Western discourse in fairness.

Scope (R3):
Our intention is to set out a research agenda and point to concrete directions one could take. Going into the specifics like solving casteist bias online is beyond the scope of our 10-page paper. We absolutely agree that caste is an important issue, and definitely warrants a paper on its own. So do many other issues we raised: fairness challenges w/ data distortions, or fairness and reservations etc. Our paper sets a research agenda for fair-ML in India that outlines open issues that need in-depth investigations, but also to outline the larger ecosystem considerations one must take into account when doing so (we will clarify).

India specific factors (R1, R3): 
Our paper discusses factors impacting fairness in India -- pronounced in India, and not necessarily unique to India (we state this). India is a globalized country. We do not wish to focus on ‘Indian’ factors in the Western imagination, and exocitize India as the ‘other’ (e.g., tropes of caste, poverty, ancient culture etc.) [ref: Edward Said and numerous decolonial authors we borrow from and cite]. Our Introducton may have contributed to the feedback, with our use of terms like ‘not limited to India alone’ (which we will revise for clarity).

Expert interviews (R2):
This method is common to many social sciences, including HCI where we come from, to understand the landscape when there are no specific systems to gain access to, and to create a systemic analysis, not specific to an intervention.

Broad (R3):
R3’s reading of the paper as broad is correct. The issues are not caused by Fair-ML factors, but impact fairness of models, fairness audit tools, and structures to turn research into reality. We mention that attempting to do Fair-ML without accounting for these broad issues may be futile or even harmful.  To articulate these sociotechnical factors, we deemed it appropriate to engage with diverse experts that work closely with marginalized communities. We will clarify these points further. 

Review #228A3 Dec 2020
Comments for author
This was a well-written, clearly presented paper.
This paper presents interview data from 36 researchers, activists and lawyers working in Indian contexts with marginalised communities. Interviews address the notion of algorithmic fairness, and the extent to which interviewees consider this feasible in light of the community groups they work with.
This is a reasonably good quality paper in terms of its empirical basis. n=36 interviews gives a solid foundation to work with (especially given the nature of the interviewees). The theoretical discussion, and arguments reached are also of a good quality. All in all, this is a good standard of paper.
Clearly written and presented - should be accessible to novice readers, and detailed enough to be of interest to people working directly in the area.
Good use of previous literature. From my own disciplinary b/g this would seem to have too much use of previous literature (194 references is about 154 more than I would expect to see!)
I am not an expert in this literature, but this paper seems to make a contribution to my adjacent knowledge of the academic literature in this area. Given the vastness and complexity of Indian society, I would welcome a clearer sense to what extent the paper can speak to 'Indian' issues, or what regional/caste nuances are being glossed over
Review #228B3 Dec 2020
Comments for author
The paper makes a relevant contribution to the study of algorithmic fairness by de-centering common practices and approaches. I am not persuaded that interviewing experts is the most appropriate method to make the case, but I think the treatment and analysis is sufficiently cogent.
Explanations of the motivation, argument, methods and results are clear and appropriate.
The paper is original in that not many scholars have attempted to achieve this analytical goal in the particular context of India (or the global south).
The paper cites abundant extant literature. It draws on appropriate bodies of work to make the case.
The argument put forth in this paper is a valuable contribution to reflections on algorithmic fairness. It helps to denaturalize common assumptions established in the field.
The contribution centers on core issues for FAccT.
Review #228C
Comments for author
Quality: The paper is well written and adequately cited. Overall, my biggest complaint is that the arguments made are very broadly centered around inequities in technology access and usage in non-western contexts, whereas the paper describes the issues as specific to shortcomings of fair machine learning in India.
Clarity: The arguments made in the paper are clear individually, but collectively, I found the paper difficult to follow. Many of the criticisms made in the paper touched on a wide array of topics: privacy, socioetechnical systems, etc. As a reader it was difficult to see how all of the issues were related to the exact same root cause -- in this case -- fair machine learning scholarship. This confusion is augmented by the breath of experts called on for interviews. They came from a number of disparate areas: "Computer Science, Activism, Law and Public Policy, etc". It would help if the scope of the criticisms in the paper were narrowed, such that more specific arguments could be made.
Originality: Although the paper is the first paper I have seen which addresses issues in the machine learning fairness scholarship that are specific to India, many of the claims made in the paper are not uniquely specific to India, and almost all of these points been cited in other works. For example, this work does a great job challenging downstream usage assumptions, and binary protected attribute assumptions: "Where Fairness Fails: Data, Algorithms, and the Limits of Anti-discrimination Discourse" by Anna Lauren Hoffman.
Significance/Impact: The paper does a great job outlining how many of the assumptions in fair machine learning are western centric, however the paper does not point to a separate body of work which remedies the issue presented. Some alternatives are mentioned, but they are often too-high level for the scope of the problems outlined in section 2. For example, "Building ties with community workers in the ML dataset collection process can be a starting point in creating high quality data, while respecting their situated knowledge. Combining observational research and dataset analysis will help us avoid misreadings of data."
Relevance: I'd say that the work is highly relevant, and that is definitely headed in the correct direction. I agree that one of the major shortcomings of the fairness literature is that the work makes many western-centric assumptions, but these assumptions are also based in power structures that appear differently everywhere, and are not necessarily unique to the western world. Underrepresentation in data being related to socioeconomic status is an issue that also occurs in the western world, and so I feel it would be helpful to frame this paper in terms of more specific Indian issues. Issues of Caste for example, are very unique to an Indian context, it would have been very helpful as a reader if the author could discuss how to better contextualize Caste, for example, in a machine learning context.



1) 
"  delay-tolerant connectivity, low cost devices, text-free interfaces, partnership with civil society  "
you can cite the Digital Green paper.
Gandhi, R., Veeraraghavan, Rajesh., Toyama, K., Ramprasad, V. Digital Green: Participatory Video for Agricultural Extension. Information Technologies & International Development, Vol. 5, Issue 1, pp1-15, Spring 2009. [PDF] 

Our idea there (though not fully developed) was breaking the idea of expertise, and making farmers as the stars (as opposed to having to rely on agri experts)maybe worth mentioning.

2) Veeraraghavan, Rajesh.Dealing with the Digital Panopticon: The Use and Subversion of ICT in an Indian Bureaucracy. IEEE/ACM Int’l Conf. on Information & Communication Technologies for Development, Cape Town, South Africa, December 2013. [PDF]
This maybe also relevant, though this is before the craze about algorithms took over. Particularly the idea of "hiding behind the computer". I had also discussed the politics of algorithms and how sometimes algorithms maybe necessary to avoid local political interference. A complex idea, but not developed :)

3) Another paper with Vivek Srinivasan (who you spoke to) where we asked the question of "direct" cash transfers, and answered. No. These tech systems needed intermediaries.
Vivek, S., Narayanan, R., Chakraborty, D., Veeraraghavan, R., Vardhan, V. Are Technology-enabled Cash Transfers Really 'Direct'? Economic and Political Weekly, July 28, 2018. [PDF] 


==> findings_table.tex <==

\begin{table*}
\small
%\centering
\begin{tabular}{p{1.5in}p{2in}p{2.5in}}
\toprule

\bottomrule
\end{tabular}
\normalsize
\caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
\end{table*}

==> subgroups_table2.tex <==
\begin{table}
\small
%\centering
\setlength{\tabcolsep}{2pt}
\begin{tabularx}{.95\linewidth}{X}
\toprule
\multicolumn{1}{c}{\bf Sub-groups, Proxies and Harms} \\
\midrule

\textbf{Caste} 
(17\% Dalits; 8\% Adivasi; 40\% Other Backward Class (OBC))\cite{CensusIndia2011} %\newline 
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
   \item \footnotesize{Societal harms: Human rights atrocities. Poverty. Land, knowledge and language battles  \cite{xaxa2011tribes, NCRBdata58:online, Twothird31:online}. }
    \item \footnotesize{Proxies: Surname. Skin tone. Occupation. Neighborhood. Language.} %\newline
    \item \footnotesize{Tech harms: Low literacy and phone ownership. Online misrepresentation \& exclusion. Accuracy gap of Facial Recognition {(FR)}. Limits of Fitzpatrick scale. Caste-based discrimination in tech {}\cite{TheCisco63:online}. }
\end{itemize}
\midrule
\textbf{Gender}
(48.5\% female)\cite{IndiaMinistryStatistics2018} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Sexual crimes. Dowry. Violence. Female infanticide.}
  \item \footnotesize{Proxies: Name. Type of labor. Mobility from home. }%
    \item \footnotesize{Tech harms: Accuracy gap in FR. Lower creditworthiness score. Recommendation algorithms favoring majority male users. Online abuse and 'racey’ content issues. Low Internet access.} 
\end{itemize}

\midrule
\textbf{Gender Identity \& Sexual Orientation}
(No official LGBTQ+ data) %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Colonial law 377 traces. Discrimination and abuse.} 
    \item \footnotesize{Proxies: Gender declaration. Name. }%
    \item \footnotesize{Tech harms: FR "outing" and accuracy. Gender binary surveillance systems in public spaces, \eg dormitories. M/F ads targeting.  Catfishing and extortion abuse attacks.}
\end{itemize}
\midrule

\textbf{Religion}
(80\% Hindu, 14\% Muslim, 6\% Christians, Sikhs, Buddhists, Jains and indigeneous) \cite{CensusIndia2011}  %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Discrimination, lynching, vigilantism, and gang-rape against Muslims and others \cite{84DeadIn98:online}.}
    \item \footnotesize{Proxies: Name. Neighborhood. Expenses. Work. Language. Clothing. } %\newline
    \item \footnotesize{Tech harms: Online stereotypes. Targeted hate speech, \eg Islamophobia. Discriminatory inferences due to lifestyle, location, appearance. Targeted Internet disruptions.} %%\newline}
\end{itemize}
\midrule

\textbf{Ability}
(5\%--8\%+ persons with disabilities) \cite{WorldBank2009Disabilities} %\newline
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Stigma. Inaccessible education, transport \& work.} 
    \item \footnotesize{Proxies: Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices.} %\newline
    \item \footnotesize{Tech harms: Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. }%\newline
\end{itemize}
\midrule


\textbf{Class}
(30\% live below poverty line; 48\% on \$2--\$10/day)\cite{Rangarajan2014Poverty} \cite{CensusIndia2011}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Poverty. Inadequate food, shelter, health, \& housing.}
    \item \footnotesize{Proxies: Spoken \& written language(s). Mother tongue. Literacy. Feature/Smart Phone Ownership. Rural vs. urban.}
    \item \footnotesize{Tech harms: Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access. }%\newline
    \end{itemize}
\midrule

\textbf{Ethnicity}
(4\% NorthEast) \cite{CensusIndia2011}
\begin{itemize}[noitemsep,leftmargin=*,topsep=2pt]
    \item \footnotesize{Societal harms: Northeastern Indians face racist slurs, discrimination, and violent attacks.}
    \item \footnotesize{Proxies: Skin tone. Facial features. Mother tongue. State. Name. }
    \item \footnotesize{Tech harms: Accuracy gap in FR. Online misrepresentation \& exclusion. Inaccurate inferences due to lifestyle, \eg migrant labor. }%\newline
\end{itemize}
\bottomrule
\end{tabularx}
\normalsize
\caption{\label{tab_subgroups} Axes of potential ML (un)fairness in India: sub-groups, marginalized groups, proxies, and harms.
}
\end{table}







% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabularx}{\textwidth}{p{1.5in} X p{2in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits; 8\% Adivasi; 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female; Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim; 7\% Other; 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on \$2-\$10/day
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day; 11\% speak English; 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. Rural vs. urban.
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule

% % \begin{comment}
% % \textbf{Region}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \midrule
% % \textbf{Gender identity}\newline
% % \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% % \tabitem 11\% speak English  \newline
% % \tabitem 69\% rural / 31 \% urban %\newline
% % %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% % &
% % \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% % &
% % \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % % & 
% % % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% % \\
% % % 
% % \bottomrule
% % \end{comment}

% \end{tabularx}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}








%VP: Backup before compressing

% \begin{table*}
% \small
% %\centering
% \setlength{\tabcolsep}{10pt}
% \begin{tabular}{p{1.5in}p{2in}p{2.5in}}
% \toprule
% \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes \\
% % \bf Sub-groups by & \bf Tech Harms and biases & \bf Proxies and attributes & \bf Fairness approaches \\
% \midrule
% \textbf{Caste} \newline
%  % Undesired contact from strangers on platforms.\newline
%  %\textit{IN: 73\%, PK: 65\%, BG: 50\%}
%   %\newline\textit{Two NGOs reported 5 incidents}
% \tabitem 17\% Dalits \newline
% \tabitem 8\% Adivasi \newline
% \tabitem 40\% OBC %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% %%NOTE: Keep the text short
% &
% \tabitem Online misrepresentation \& lack of representation. Accuracy of Facial Recognition {(FR)}.
% %  \newline
% & 
% \tabitem Surname. Skin tone. Occupation. Neighborhood %\newline
% % & 
% % \tabitem Testing, augmenting model data with surname perturbation data. \newline 
% % \tabitem Rater bias training. \newline 
% % \tabitem Semantic analysis. \newline 
% % \tabitem Quick check for casteist words, \eg{'mahar'}. 
% \\
% \midrule
% \textbf{Gender}\newline
% \tabitem 48.5\% female \newline
% \tabitem Variable count LGBTQ+ %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Accuracy of FR. Classified as less credit worthy. Shown popular male content. 'Racey’ content and its implications. 
% &
% \tabitem Type of labor. Mobility. Gender declaration. Name. %
% % & 
% % \tabitem Non-binary gender labels. \newline
% % \tabitem Mechanisms to correct gender identifiers in data. \newline
% % \tabitem Testing, augmenting model data with m/f perturbation data. 
% \\
% \midrule
% \textbf{Religion}\newline
% \tabitem 13\% Muslim \newline
% \tabitem 7\% Other \newline
% \tabitem 80\% Hindu %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Online representation and stereotypes. Toxicity and hate speech from Islamophobia. High-stakes AI inferences.  %%\newline
% &
% \tabitem Name, Neighborhood, Expenditures, Occupation, Language, Clothing (\eg head covering, direction dhoti is tied) %\newline
% % & 
% % \tabitem Adversarial tests. \newline
% % \tabitem Diversity of representation. \newline
% % \tabitem Semantic analysis. \newline
% % \tabitem Rater bias training. \newline
%  \\
% \midrule
% \textbf{Ability}\newline
% \tabitem 4\% - 8\%+ PWD %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Assumed homogeneity in physical, mental presentation. Paternalistic words and images. No accessibility mandate. %\newline
% &
% \tabitem Non-normative facial features, speech patterns, body shape \& movements. Use of assistive devices. %\newline
% % & 
% % \tabitem Alt options for biometric inputs. \newline
% % \tabitem Robust speech \& language understanding models. \newline
% % \tabitem Adherence to SIG ACCESS guidelines for PWD terminology. 
% \\
% \midrule
% \textbf{Class}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% %\multicolumn{4}{c}{\textit{Participant reports are likely to be low estimates,because of stigma and trauma with discussing abuse. Among only 4 NGOs, we heard of 15 distinct incidents.}} \\
% \bottomrule
% \begin{comment}
% \textbf{Region}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \midrule
% \textbf{Gender identity}\newline
% \tabitem 30\% live below poverty line; \newline 48\% on $2-$10/day \newline
% \tabitem 11\% speak English  \newline
% \tabitem 69\% rural / 31 \% urban %\newline
% %\tabitem \textit{IN: 7\%, PK: 77\%, BG: 43\%}\newline
% &
% \tabitem Linguistic bias towards mainstream languages. Model bias towards middle class users. Limited or lack of internet access.%\newline
% &
% \tabitem Spoken language(s). Mother tongue. Written language(s). Literacy. Feature / Smart Phone Ownership. %\newline
% % & 
% % \tabitem Inclusion of Indic languages in consent, applications. \newline
% % \tabitem Avoiding practice  of “free” apps that profit on user data collection. 
% \\
% % 
% \bottomrule
% \end{comment}
% \end{tabular}
% \normalsize
% \caption{Sub-groups, proxies, and measurements in model fairness in India.\label{tab_subgroups}}
% \end{table*}


